Retrieval-Seeded Diffusion for Semantic Flow Models

Diffusion models are trained to map a source distribution (usually, a Gaussian) to a target distribution (say, of natural images). The Gaussian distribution is chosen because it is easy to sample from, and the diffusion process is often guided by a text prompt in order to achieve a specific outcome. A recent line of text-to-image models operates in semantic latent spaces rather than a pixel compression one, so that nearby latents share content rather than appearance, and it is these semantic models that we focus on. Often, the images we want belong to the domain of a specific dataset, such as photographs, anime or paintings, yet sampling still starts from the same Gaussian, which takes neither the prompt nor the dataset into account. We propose a method that generates images more similar to the dataset's domain, in fewer steps, by enhancing the Gaussian using the dataset, and call this approach Retrieval-Seeded Diffusion, or RSD. Specifically, we store a semantic latents dataset of captioned images. Given a new text prompt, we find its nearest neighbours in the text embedding space, use them to retrieve their semantic latent image representation counterparts, and use the mean of the semantic latent image vectors to guide the initial seed for the diffusion model. Relying on a dataset requires no training and a new dataset can always be introduced or updated. Experiments on three frozen semantic backbones, Scale-RAE, SVG-T2I and SeFi-Image, and three retrieved datasets, show that RSD lowers FID to the target dataset in eight of nine settings, by up to 57%, at 6.25x fewer sampling steps, with comparable prompt alignment.

==> figures/attribution/fig_attribution.tex <==
\begin{figure}[!h]
  \centering
  \input{figures/attribution/values}%
  \newcommand{\attrside}{0.17\linewidth}%
  \newcommand{\attrgap}{0.012\linewidth}%
  \newcommand{\attrrowgap}{12pt}%
  \newcommand{\attrmu}{0.07\linewidth}%
  \newcommand{\attrarrow}{0.045\linewidth}%
  \newcommand{\attrboxw}{0.12\linewidth}%
  \newcommand{\attrbarsep}{1.8pt}%
  \newcommand{\attrbarh}{2pt}%
  \newcommand{\attrframe}{0.3pt}%
  \newcommand{\attrpctfont}{\usefont{T1}{ppl}{m}{it}}%
  \newcommand{\attrfont}{\scriptsize}%
  \newcommand{\attrpromptfont}{\footnotesize}%
  \newcommand{\attrpromptw}{0.82\linewidth}%
  \newcommand{\attrpromptlift}{17pt}%
  \newcommand{\attrpromptfill}{black!2.5}%
  \newcommand{\attrretpad}{3pt}%
  \newcommand{\attrretdraw}{black!25}%
  \newcommand{\attrsnowr}{3.1pt}%
  \definecolor{attrsnow}{HTML}{5BA4E6}%
  \newcommand{\attrdotsep}{4pt}%
  \newcommand{\attrimg}[1]{\includegraphics[width=\attrside,height=\attrside]{figures/attribution/img/#1}}%
  \ifdefined\figcachebegin\figcachebegin{attribution}\fi
  \begin{tikzpicture}[panel/.style={inner sep=0pt, outer sep=0pt},
                      pct/.style={inner sep=0pt, font=\attrfont\attrpctfont},
                      flow/.style={black!55, line width=0.8pt, -{Stealth[length=4.5pt, width=5pt]}}]
    \node[panel, anchor=south west] (n3) at (0,0) {\attrimg{nb3.jpg}};
    \node[panel, anchor=west] (n4) at ($(n3.east)+(\attrgap,0)$) {\attrimg{nb4.jpg}};
    \node[panel, anchor=south] (n1) at ($(n3.north)+(0,\attrrowgap)$) {\attrimg{nb1.jpg}};
    \node[panel, anchor=west] (n2) at ($(n1.east)+(\attrgap,0)$) {\attrimg{nb2.jpg}};
    \coordinate (gmid) at ($(n2.south east)!0.5!(n4.north east)$);
    \node[panel, anchor=west] (anc) at ($(gmid)+(\attrmu,0)$) {\attrimg{anchor.jpg}};
    \node[draw=black!60, fill=otherblue!6, rounded corners=3pt, line width=0.6pt, font=\small,
          minimum width=\attrboxw, minimum height=0.62*\attrside]
      (model) at ($(anc.east)+(\attrarrow+0.5*\attrboxw,0)$) {\raisebox{-2pt}{$\vv_\vtheta$}};
    \begin{scope}[shift={($(model.north west)+(2.2pt+\attrsnowr,-2.2pt-\attrsnowr)$)}, attrsnow, line width=0.45pt, line cap=round]
      \foreach \a in {0,60,...,300} {
        \draw (0,0) -- (\a:\attrsnowr);
        \draw ($(\a:0.55*\attrsnowr)$) -- +(\a+40:0.38*\attrsnowr) ($(\a:0.55*\attrsnowr)$) -- +(\a-40:0.38*\attrsnowr);}
    \end{scope}
    \node[panel, anchor=west] (out) at ($(model.east)+(\attrarrow,0)$) {\attrimg{out.jpg}};
    \foreach \n in {out,anc,n1,n2,n3,n4}
      \draw[black, line width=\attrframe] (\n.south west) rectangle (\n.north east);
    \foreach \i/\n in {1/A,2/B,3/C,4/D} {
      \fill[black!10] ($(n\i.south west)+(0,-\attrbarsep)$) rectangle ($(n\i.south east)+(0,-\attrbarsep-\attrbarh)$);
      \fill[otherblue] ($(n\i.south west)+(0,-\attrbarsep)$)
                       rectangle ($(n\i.south west)+(\csname attrw\n\endcsname*\attrside,-\attrbarsep-\attrbarh)$);
      \node[pct, anchor=north] at ($(n\i.south)+(0,-\attrbarsep-\attrbarh-1.5pt)$) {\csname attrp\n\endcsname\%};}
    \node[pct, anchor=north, text=black!55] (more) at ($(n3.south east)!0.5!(n4.south west)+(0,-\attrbarsep-\attrbarh-9pt)$)
      {$+$\attrrest\ more};
    \foreach \d in {1,2,3}
      \fill[black!\the\numexpr 55-12*\d\relax] ($(more.west)+(-\d*\attrdotsep+0.5*\attrdotsep-2pt,0.2ex)$) circle (1.1pt);
    \begin{scope}[on background layer]
      \node[fit=(n1)(n2)(n3)(n4)(more), inner sep=\attrretpad, fill=\attrpromptfill, draw=\attrretdraw, line width=0.5pt,
            rounded corners=6pt] (ret) {};
    \end{scope}
    \draw[flow] (gmid -| ret.east) -- node[above, font=\attrfont, inner sep=2pt] {$\vmu$} (anc);
    \draw[flow] (anc) -- (model);
    \draw[flow] (model) -- (out);
    \node[pct, anchor=north, text=black!55] at ($(anc.south)+(0,-\attrbarsep-0.5pt)$) {decoded anchor};
    \node[anchor=north, inner sep=0pt, font=\attrfont] at ($(out.south)+(0,-\attrbarsep-0.5pt)$)
      {\textcolor{otherblue}{\textbf{\method{} (ours)}}};
    \coordinate (brkM) at (ret.north);
    \path let \p1 = (ret.west), \p2 = (out.east), \p3 = (n1.north) in%
      node[inner ysep=2.5pt, inner xsep=5pt, anchor=south, font=\attrpromptfont, fill=\attrpromptfill, draw=black!10,
           line width=0.5pt, rounded corners=6pt, text width=\attrpromptw, align=center]
        (prompt) at ({0.5*(\x1+\x2)}, {\y3+\attrpromptlift}) {\gridprompt{\attrprompt}};
    \draw[flow] (prompt.south -| brkM) -- node[right, pct, text=black!55, inner sep=2pt] {Retrieved} (brkM);
    \draw[flow] (prompt.south -| model.north) -- (model.north);
  \end{tikzpicture}%
  \ifdefined\figcacheend\figcacheend\fi
  \caption{\textbf{Attribution.} A generated image (right) and the four retrieved images (left) that contributed most to its anchor with their percentages. The anchor is decoded (middle) to show what it looks like in the image space.
  }
  \label{fig:attribution}
\end{figure}


==> figures/attribution/values.tex <==
\newcommand{\attrwA}{0.6004}%
\newcommand{\attrpA}{60.0}%
\newcommand{\attrwB}{0.1240}%
\newcommand{\attrpB}{12.4}%
\newcommand{\attrwC}{0.1012}%
\newcommand{\attrpC}{10.1}%
\newcommand{\attrwD}{0.0573}%
\newcommand{\attrpD}{5.7}%
\newcommand{\attrtop}{88}%
\newcommand{\attrrest}{46}%
\newcommand{\attrk}{50}%
\newcommand{\attrprompt}{a person skiing through the snow near some trees toward a sunset}%
\newcommand{\attroursN}{8}%
\newcommand{\attrbaseN}{50}%


==> figures/density/fig_density.tex <==
\begin{figure}[t]
  \centering
  \input{figures/density/values}%
  \newcommand{\dkw}{0.37\linewidth}%
  \newcommand{\dkh}{0.30\linewidth}%
  \newcommand{\dkbar}{4pt}%
  \newcommand{\dkgap}{0.4pt}%
  \newcommand{\dkfont}{\scriptsize}%
  \newcommand{\dklegfont}{\footnotesize}%
  \definecolor{dkbase}{HTML}{EB6834}%
  \definecolor{dkours}{HTML}{2A78D6}%
  \newcommand{\dkv}[4]{\csname density@#1@#2@#3#4\endcsname}%
  \pgfplotsset{dkaxis/.style={ybar, bar width=\dkbar, width=\dkw, height=\dkh,
      scale only axis, xmin=-0.6, xmax=4.6, xtick={0,...,4}, xticklabels={},
      clip=false, ymin=0, axis x line*=bottom, axis y line*=left,
      ymajorgrids, grid style={black!12, line width=0.3pt},
      tick label style={font=\dkfont}, label style={font=\dkfont},
      every axis y label/.style={at={(ticklabel* cs:1)}, anchor=south, yshift=2pt, font=\dkfont},
      xlabel={dense $\rightarrow$ sparse}, xlabel style={yshift=10pt},
      major x tick style={draw=none}},
    dkerr/.style={error bars/.cd, y dir=both, y explicit,
      error bar style={line width=0.4pt, black!75},
      error mark options={rotate=90, mark size=1pt, line width=0.4pt, black!75}},
    dkswatch/.style={legend image code/.code={\fill[#1] (0pt,-2.5pt) rectangle (8pt,3pt);}}}%
  \newcommand{\dkpanel}[4]{%
    \begin{tikzpicture}
      \begin{axis}[dkaxis, ylabel={FID-1k $\downarrow$}, #3]
        #4
        \foreach \a/\c/\s in {base/dkbase/-0.5, ours/dkours/0.5} {
          \edef\dkplot{\noexpand\addplot[fill=\c, draw=none, bar shift=\s*(\dkbar+\dkgap), dkerr]
            coordinates {
              (0,\dkv{#1}{\a}{0}{}) +- (0,\dkv{#1}{\a}{0}{@ci})
              (1,\dkv{#1}{\a}{1}{}) +- (0,\dkv{#1}{\a}{1}{@ci})
              (2,\dkv{#1}{\a}{2}{}) +- (0,\dkv{#1}{\a}{2}{@ci})
              (3,\dkv{#1}{\a}{3}{}) +- (0,\dkv{#1}{\a}{3}{@ci})
              (4,\dkv{#1}{\a}{4}{}) +- (0,\dkv{#1}{\a}{4}{@ci})};}\dkplot}
        \node[anchor=south east, font=\dkfont, inner sep=1pt, yshift=2pt] at (rel axis cs:1,1) {#2};
      \end{axis}
    \end{tikzpicture}}%
  \dkpanel{rae}{Scale-RAE}{legend to name=dklegend, legend columns=2,
      legend style={draw=none, font=\dklegfont, /tikz/every even column/.append style={column sep=6pt}}}%
    {\addlegendimage{dkswatch=dkbase}\addlegendentry{Baseline}
     \addlegendimage{dkswatch=dkours}\addlegendentry{\method}}\hfill
  \dkpanel{svg}{SVG-T2I}{}{}
  \\[2pt]
  \pgfplotslegendfromname{dklegend}
  \caption{\textbf{The gain across corpus density.} FID-1k of each backbone's released sampler and of
    \method, with the $5{,}000$ prompts split into five bins of about $1{,}000$ by
    the similarity of their nearest corpus caption, each bin scored against the
    val2017 photos its prompts describe.
    }
  \label{fig:density}
\end{figure}


==> figures/density/values.tex <==
\expandafter\def\csname density@rae@base@0\endcsname{65.236}%
\expandafter\def\csname density@rae@base@0@ci\endcsname{1.962}%
\expandafter\def\csname density@rae@ours@0\endcsname{57.533}%
\expandafter\def\csname density@rae@ours@0@ci\endcsname{1.854}%
\expandafter\def\csname density@rae@base@1\endcsname{65.225}%
\expandafter\def\csname density@rae@base@1@ci\endcsname{1.897}%
\expandafter\def\csname density@rae@ours@1\endcsname{60.109}%
\expandafter\def\csname density@rae@ours@1@ci\endcsname{2.054}%
\expandafter\def\csname density@rae@base@2\endcsname{69.151}%
\expandafter\def\csname density@rae@base@2@ci\endcsname{2.283}%
\expandafter\def\csname density@rae@ours@2\endcsname{62.642}%
\expandafter\def\csname density@rae@ours@2@ci\endcsname{2.107}%
\expandafter\def\csname density@rae@base@3\endcsname{72.431}%
\expandafter\def\csname density@rae@base@3@ci\endcsname{2.107}%
\expandafter\def\csname density@rae@ours@3\endcsname{64.850}%
\expandafter\def\csname density@rae@ours@3@ci\endcsname{1.980}%
\expandafter\def\csname density@rae@base@4\endcsname{74.634}%
\expandafter\def\csname density@rae@base@4@ci\endcsname{2.103}%
\expandafter\def\csname density@rae@ours@4\endcsname{68.167}%
\expandafter\def\csname density@rae@ours@4@ci\endcsname{2.089}%
\expandafter\def\csname density@svg@base@0\endcsname{61.315}%
\expandafter\def\csname density@svg@base@0@ci\endcsname{2.164}%
\expandafter\def\csname density@svg@ours@0\endcsname{53.565}%
\expandafter\def\csname density@svg@ours@0@ci\endcsname{1.737}%
\expandafter\def\csname density@svg@base@1\endcsname{60.650}%
\expandafter\def\csname density@svg@base@1@ci\endcsname{2.107}%
\expandafter\def\csname density@svg@ours@1\endcsname{54.691}%
\expandafter\def\csname density@svg@ours@1@ci\endcsname{1.862}%
\expandafter\def\csname density@svg@base@2\endcsname{64.172}%
\expandafter\def\csname density@svg@base@2@ci\endcsname{2.101}%
\expandafter\def\csname density@svg@ours@2\endcsname{57.729}%
\expandafter\def\csname density@svg@ours@2@ci\endcsname{1.886}%
\expandafter\def\csname density@svg@base@3\endcsname{66.415}%
\expandafter\def\csname density@svg@base@3@ci\endcsname{2.062}%
\expandafter\def\csname density@svg@ours@3\endcsname{59.392}%
\expandafter\def\csname density@svg@ours@3@ci\endcsname{1.805}%
\expandafter\def\csname density@svg@base@4\endcsname{67.408}%
\expandafter\def\csname density@svg@base@4@ci\endcsname{1.958}%
\expandafter\def\csname density@svg@ours@4\endcsname{62.255}%
\expandafter\def\csname density@svg@ours@4@ci\endcsname{1.964}%


==> figures/div_grid/fig_div_grid.tex <==
\input{figures/div_grid/values}%
\begin{figure*}[t]
  \centering
  \newcommand{\dglabw}{10pt}%
  \newcommand{\dgin}{1pt}%
  \newcommand{\dgout}{5pt}%
  \newcommand{\dgpromptsep}{1.5pt}%
  \newcommand{\dgrowsep}{4pt}%
  \newcommand{\dgheadsep}{2pt}%
  \newcommand{\dgpromptfont}{\scriptsize}%
  \newcommand{\dgheadfont}{\footnotesize}%
  \newcommand{\dglabfont}{\scriptsize}%
  \newcommand{\dgframe}{0.3pt}%
  \definecolor{dgbase}{HTML}{EB6834}%
  \definecolor{dgrmg}{HTML}{4E9F5B}%
  \setlength{\fboxsep}{0pt}\setlength{\fboxrule}{\dgframe}%
  \ifdefined\dgpw\else\newlength{\dgpw}\newlength{\dggrw}\newlength{\dgrw}\fi
  \ifdefined\dgbh\else\newlength{\dgbh}\fi
  \setlength{\dgpw}{\linewidth}\addtolength{\dgpw}{-\dglabw}%
  \addtolength{\dgpw}{-2\dimexpr\dgout\relax}\addtolength{\dgpw}{-3\dimexpr\dgin\relax}\divide\dgpw by 6
  \setlength{\dggrw}{2\dgpw}\addtolength{\dggrw}{\dgin}%
  \setlength{\dgbh}{2\dgpw}\addtolength{\dgbh}{\dgin}%
  \setlength{\dgrw}{3\dggrw}\addtolength{\dgrw}{2\dimexpr\dgout\relax}%
  \newcommand{\dgimg}[2]{\fbox{\includegraphics[width=\dimexpr\dgpw-2\fboxrule\relax]{figures/div_grid/img/#1/#2.jpg}}}%
  \newcommand{\dggroup}[2]{\parbox[b]{\dggrw}{\offinterlineskip
    \hbox{\dgimg{#1}{#2_0}\hspace{\dgin}\dgimg{#1}{#2_1}}\vskip\dgin
    \hbox{\dgimg{#1}{#2_2}\hspace{\dgin}\dgimg{#1}{#2_3}}}}%
  \newcommand{\dglab}[1]{\parbox[b][\dgbh][c]{\dglabw}{\centering\rotatebox{90}{\dglabfont #1}}}%
  \newcommand{\dgrow}[2]{\noindent\dglab{#2}\hfill\begin{minipage}[b]{\dgrw}\centering
      {\dgpromptfont\gridprompt{\csname divgrid@#1\endcsname}\par}\vspace{\dgpromptsep}%
      \dggroup{#1}{base}\hspace{\dgout}\dggroup{#1}{rmg}\hspace{\dgout}\dggroup{#1}{ours}%
    \end{minipage}\par\vspace{\dgrowsep}}%
  \newcommand{\dghead}{\noindent\hspace*{\dglabw}\hfill\begin{minipage}[b]{\dgrw}\dgheadfont
      \parbox[b]{\dggrw}{\centering\color{dgbase}Baseline}\hspace{\dgout}%
      \parbox[b]{\dggrw}{\centering\color{dgrmg}RMG}\hspace{\dgout}%
      \parbox[b]{\dggrw}{\centering\color{otherblue}\textbf{\method{} (ours)}}%
    \end{minipage}\par\vspace{\dgheadsep}}%
  \dghead
  \dgrow{r2854}{Scale-RAE}
  \dgrow{r207}{SeFi-Image}
  \dgrow{r2552}{SVG-T2I}
  \vspace{-\dgrowsep}
  \caption{\textbf{Per-prompt diversity on COCO.} Four samples of each prompt, each from a different noise draw, by
    the released sampler with $50$ steps, RMG with $20$ and \method with $8$.}
  \label{fig:div_grid}
\end{figure*}


==> figures/div_grid/values.tex <==
\expandafter\def\csname divgrid@r2854\endcsname{A red and white boat floating along a river.}%
\expandafter\def\csname divgrid@r207\endcsname{A man in a suit is wearing a lit up tie.}%
\expandafter\def\csname divgrid@r2552\endcsname{A large white clock tower filled with light.}%


==> figures/diversity_bars/fig_diversity_bars.tex <==
\begin{figure}[t]
  \centering
  \input{figures/diversity_bars/values}%
  \newcommand{\dbw}{0.22\linewidth}%
  \newcommand{\dbh}{0.17\linewidth}%
  \newcommand{\dbbar}{3.6pt}%
  \newcommand{\dbgap}{0.4pt}%
  \newcommand{\dbfont}{\scriptsize}%
  \newcommand{\dbxfont}{\tiny}%
  \newcommand{\dblegfont}{\footnotesize}%
  \definecolor{dbbase}{HTML}{EB6834}%
  \definecolor{dbrmg}{HTML}{4E9F5B}%
  \definecolor{dbours}{HTML}{2A78D6}%
  \newcommand{\dbv}[3]{\csname divbars@#1@#2@#3@rel\endcsname}%
  \pgfplotsset{dbaxis/.style={ybar, bar width=\dbbar, width=\dbw, height=\dbh,
      scale only axis, symbolic x coords={Scale-RAE,SVG-T2I,SeFi}, xtick={Scale-RAE,SVG-T2I,SeFi},
      enlarge x limits={abs=7pt}, clip=false, enlarge y limits={abs=1.5}, max space between ticks=14,
      axis x line*=bottom, axis y line*=left, ymajorgrids, grid style={black!12, line width=0.3pt},
      tick label style={font=\dbfont}, label style={font=\dbfont}, title style={font=\dbfont, yshift=-5pt},
      x tick label style={font=\dbxfont, rotate=35, anchor=north east, inner sep=1pt},
      major x tick style={draw=none},
      extra y ticks={0}, extra y tick labels={},
      extra y tick style={grid=major, major grid style={dbbase, dashed, line width=0.7pt}, major tick length=0pt}}}%
  \newcommand{\dbpanel}[4]{%
    \begin{tikzpicture}[baseline=(dbax.south)]
      \begin{axis}[dbaxis, name=dbax, title={#2}, #3]
        #4
        \foreach \a/\c/\s in {rmg/dbrmg/-0.5, ours/dbours/0.5} {
          \edef\dbplot{\noexpand\addplot[fill=\c, draw=none, bar shift=\s*(\dbbar+\dbgap)]
            coordinates {(Scale-RAE,\dbv{rae}{\a}{#1}) (SVG-T2I,\dbv{svg}{\a}{#1}) (SeFi,\dbv{sefi}{\a}{#1})};}\dbplot}
      \end{axis}
    \end{tikzpicture}}%
  \dbpanel{lpips}{LPIPS}{ylabel={Change (\%)}, ylabel style={yshift=-4pt}, legend to name=dblegend, legend columns=3,
      legend style={draw=none, font=\dblegfont, inner sep=0pt, /tikz/every even column/.append style={column sep=5pt}}}%
    {\addlegendimage{legend image code/.code={\draw[dbbase, dashed, line width=0.7pt] (0pt,0pt) -- (10pt,0pt);}}\addlegendentry{Released sampler}
     \addlegendimage{legend image code/.code={\fill[dbrmg] (0pt,-2.5pt) rectangle (8pt,3pt);}}\addlegendentry{RMG}
     \addlegendimage{legend image code/.code={\fill[dbours] (0pt,-2.5pt) rectangle (8pt,3pt);}}\addlegendentry{\method}}\hfill
  \dbpanel{dreamsim}{DreamSim}{}{}\hfill
  \dbpanel{vendi}{Vendi}{}{}
  \\[0pt]
  \pgfplotslegendfromname{dblegend}
  \caption{\textbf{Per-prompt diversity relative to the released sampler.} Three measures of how much the
    four samples of a prompt differ, over $1{,}000$ prompts: their mean pairwise LPIPS and DreamSim distances
    and their Vendi score, higher is more diverse. Each bar is the change of \method or
    RMG~\cite{curvo2026follow} from the backbone's released sampler
    (dashed). \method keeps or raises the released sampler's diversity in almost all cases, while RMG lowers it
    on Scale-RAE.
    }
  \label{fig:diversity_bars}
\end{figure}


==> figures/diversity_bars/values.tex <==
\expandafter\def\csname divbars@rae@base@lpips\endcsname{0.6642}%
\expandafter\def\csname divbars@rae@base@lpips@ci\endcsname{0.0041}%
\expandafter\def\csname divbars@rae@base@lpips@rel\endcsname{0.000}%
\expandafter\def\csname divbars@rae@base@dreamsim\endcsname{0.3851}%
\expandafter\def\csname divbars@rae@base@dreamsim@ci\endcsname{0.0068}%
\expandafter\def\csname divbars@rae@base@dreamsim@rel\endcsname{0.000}%
\expandafter\def\csname divbars@rae@base@vendi\endcsname{2.6341}%
\expandafter\def\csname divbars@rae@base@vendi@ci\endcsname{0.0326}%
\expandafter\def\csname divbars@rae@base@vendi@rel\endcsname{0.000}%
\expandafter\def\csname divbars@rae@rmg@lpips\endcsname{0.5933}%
\expandafter\def\csname divbars@rae@rmg@lpips@ci\endcsname{0.0050}%
\expandafter\def\csname divbars@rae@rmg@lpips@rel\endcsname{-10.674}%
\expandafter\def\csname divbars@rae@rmg@dreamsim\endcsname{0.2863}%
\expandafter\def\csname divbars@rae@rmg@dreamsim@ci\endcsname{0.0055}%
\expandafter\def\csname divbars@rae@rmg@dreamsim@rel\endcsname{-25.656}%
\expandafter\def\csname divbars@rae@rmg@vendi\endcsname{2.2940}%
\expandafter\def\csname divbars@rae@rmg@vendi@ci\endcsname{0.0279}%
\expandafter\def\csname divbars@rae@rmg@vendi@rel\endcsname{-12.911}%
\expandafter\def\csname divbars@rae@ours@lpips\endcsname{0.6573}%
\expandafter\def\csname divbars@rae@ours@lpips@ci\endcsname{0.0042}%
\expandafter\def\csname divbars@rae@ours@lpips@rel\endcsname{-1.039}%
\expandafter\def\csname divbars@rae@ours@dreamsim\endcsname{0.4007}%
\expandafter\def\csname divbars@rae@ours@dreamsim@ci\endcsname{0.0066}%
\expandafter\def\csname divbars@rae@ours@dreamsim@rel\endcsname{4.051}%
\expandafter\def\csname divbars@rae@ours@vendi\endcsname{2.7042}%
\expandafter\def\csname divbars@rae@ours@vendi@ci\endcsname{0.0319}%
\expandafter\def\csname divbars@rae@ours@vendi@rel\endcsname{2.661}%
\expandafter\def\csname divbars@svg@base@lpips\endcsname{0.6521}%
\expandafter\def\csname divbars@svg@base@lpips@ci\endcsname{0.0041}%
\expandafter\def\csname divbars@svg@base@lpips@rel\endcsname{0.000}%
\expandafter\def\csname divbars@svg@base@dreamsim\endcsname{0.3362}%
\expandafter\def\csname divbars@svg@base@dreamsim@ci\endcsname{0.0058}%
\expandafter\def\csname divbars@svg@base@dreamsim@rel\endcsname{0.000}%
\expandafter\def\csname divbars@svg@base@vendi\endcsname{2.3837}%
\expandafter\def\csname divbars@svg@base@vendi@ci\endcsname{0.0309}%
\expandafter\def\csname divbars@svg@base@vendi@rel\endcsname{0.000}%
\expandafter\def\csname divbars@svg@rmg@lpips\endcsname{0.6260}%
\expandafter\def\csname divbars@svg@rmg@lpips@ci\endcsname{0.0040}%
\expandafter\def\csname divbars@svg@rmg@lpips@rel\endcsname{-4.002}%
\expandafter\def\csname divbars@svg@rmg@dreamsim\endcsname{0.3302}%
\expandafter\def\csname divbars@svg@rmg@dreamsim@ci\endcsname{0.0054}%
\expandafter\def\csname divbars@svg@rmg@dreamsim@rel\endcsname{-1.785}%
\expandafter\def\csname divbars@svg@rmg@vendi\endcsname{2.4297}%
\expandafter\def\csname divbars@svg@rmg@vendi@ci\endcsname{0.0289}%
\expandafter\def\csname divbars@svg@rmg@vendi@rel\endcsname{1.930}%
\expandafter\def\csname divbars@svg@ours@lpips\endcsname{0.6575}%
\expandafter\def\csname divbars@svg@ours@lpips@ci\endcsname{0.0036}%
\expandafter\def\csname divbars@svg@ours@lpips@rel\endcsname{0.828}%
\expandafter\def\csname divbars@svg@ours@dreamsim\endcsname{0.3697}%
\expandafter\def\csname divbars@svg@ours@dreamsim@ci\endcsname{0.0055}%
\expandafter\def\csname divbars@svg@ours@dreamsim@rel\endcsname{9.964}%
\expandafter\def\csname divbars@svg@ours@vendi\endcsname{2.5671}%
\expandafter\def\csname divbars@svg@ours@vendi@ci\endcsname{0.0301}%
\expandafter\def\csname divbars@svg@ours@vendi@rel\endcsname{7.694}%
\expandafter\def\csname divbars@sefi@base@lpips\endcsname{0.6495}%
\expandafter\def\csname divbars@sefi@base@lpips@ci\endcsname{0.0049}%
\expandafter\def\csname divbars@sefi@base@lpips@rel\endcsname{0.000}%
\expandafter\def\csname divbars@sefi@base@dreamsim\endcsname{0.3230}%
\expandafter\def\csname divbars@sefi@base@dreamsim@ci\endcsname{0.0087}%
\expandafter\def\csname divbars@sefi@base@dreamsim@rel\endcsname{0.000}%
\expandafter\def\csname divbars@sefi@base@vendi\endcsname{2.2592}%
\expandafter\def\csname divbars@sefi@base@vendi@ci\endcsname{0.0395}%
\expandafter\def\csname divbars@sefi@base@vendi@rel\endcsname{0.000}%
\expandafter\def\csname divbars@sefi@rmg@lpips\endcsname{0.6631}%
\expandafter\def\csname divbars@sefi@rmg@lpips@ci\endcsname{0.0043}%
\expandafter\def\csname divbars@sefi@rmg@lpips@rel\endcsname{2.094}%
\expandafter\def\csname divbars@sefi@rmg@dreamsim\endcsname{0.3870}%
\expandafter\def\csname divbars@sefi@rmg@dreamsim@ci\endcsname{0.0083}%
\expandafter\def\csname divbars@sefi@rmg@dreamsim@rel\endcsname{19.814}%
\expandafter\def\csname divbars@sefi@rmg@vendi\endcsname{2.6542}%
\expandafter\def\csname divbars@sefi@rmg@vendi@ci\endcsname{0.0395}%
\expandafter\def\csname divbars@sefi@rmg@vendi@rel\endcsname{17.484}%
\expandafter\def\csname divbars@sefi@ours@lpips\endcsname{0.6617}%
\expandafter\def\csname divbars@sefi@ours@lpips@ci\endcsname{0.0043}%
\expandafter\def\csname divbars@sefi@ours@lpips@rel\endcsname{1.878}%
\expandafter\def\csname divbars@sefi@ours@dreamsim\endcsname{0.3820}%
\expandafter\def\csname divbars@sefi@ours@dreamsim@ci\endcsname{0.0075}%
\expandafter\def\csname divbars@sefi@ours@dreamsim@rel\endcsname{18.266}%
\expandafter\def\csname divbars@sefi@ours@vendi\endcsname{2.6061}%
\expandafter\def\csname divbars@sefi@ours@vendi@ci\endcsname{0.0380}%
\expandafter\def\csname divbars@sefi@ours@vendi@rel\endcsname{15.355}%


==> figures/fid_vs_nfe/fid_vs_nfe.tex <==
\begin{figure*}[t]
  \centering
  \newcommand{\fvnw}{0.32}%
  \newcommand{\fvnlab}[1]{{\small #1}}%
  \newcommand{\fvnpanel}[2]{\parbox[b]{\fvnw\linewidth}{\centering\fvnlab{#1}\\[1pt]%
    \includegraphics{figures/fid_vs_nfe/fid_vs_nfe_#2.pdf}}}%
  \includegraphics{figures/fid_vs_nfe/fid_vs_nfe_legend.pdf}\\[2pt]
  \fvnpanel{Scale-RAE}{scale_rae}\hfill\fvnpanel{SVG-T2I}{svg_t2i}\hfill\fvnpanel{SeFi-Image}{sefi}
  \caption{\textbf{FID against sampling steps.} \method, RMG and each backbone's released sampler on COCO
  across numbers of steps. The dashed line is the released sampler at its full $50$ steps. Large markers show each method's released settings.}
  \label{fig:fid_vs_nfe}
\end{figure*}


==> figures/keff_backbones/fig_keff_backbones.tex <==
\begin{figure}[t]
  \centering
  \input{figures/keff_backbones/values}%
  \input{figures/div_keff/style}%
  \ifdefined\figcachebegin\figcachebegin{keff_backbones}\fi
  \dklegend{5}{\addlegendimage{dk base}\addlegendentry{Released sampler}
    \addlegendimage{dk lpips}\addlegendentry{LPIPS}
    \addlegendimage{dk dreamsim}\addlegendentry{DreamSim}
    \addlegendimage{dk vendi}\addlegendentry{Vendi}
    \addlegendimage{dk fid}\addlegendentry{FID}}
  \\[1pt]
  \dkpanel{svg}{dkdiv}{title={SVG-T2I}, xlabel={}, ylabel={Diversity $\uparrow$ (\%)}, ymin=-14, ymax=24, ytick={-10,0,10,20}}%
    {\dkplot{svg}{lpips}\dkplot{svg}{dreamsim}\dkplot{svg}{vendi}}{}{$\tau = 0.02$}\hfill
  \dkpanel{svg}{dkqual}{title={SVG-T2I}, xlabel={}, ylabel={FID $\downarrow$ (\%)}, ymin=-30, ymax=4, ytick={-30,-20,-10,0}}%
    {\dkplot{svg}{fid}}{}{$\tau = 0.02$}
  \\[2pt]
  \dkpanel{sefi}{dkdiv}{title={SeFi-Image}, ylabel={Diversity $\uparrow$ (\%)}, ymin=-14, ymax=24, ytick={-10,0,10,20}}%
    {\dkplot{sefi}{lpips}\dkplot{sefi}{dreamsim}\dkplot{sefi}{vendi}}{}{$\tau = 0.02$}\hfill
  \dkpanel{sefi}{dkqual}{title={SeFi-Image}, ylabel={FID $\downarrow$ (\%)}, ymin=-30, ymax=4, ytick={-30,-20,-10,0}}%
    {\dkplot{sefi}{fid}}{}{$\tau = 0.02$}
  \ifdefined\figcacheend\figcacheend\fi
  \caption{\textbf{Diversity and FID against the effective number of neighbours on SVG-T2I and SeFi-Image.}
    As \cref{fig:div_keff,fig:div_keff_supp}, for \method as $\tau$ varies at $k = 50$, each as the change
    from the released sampler (dashed). SVG-T2I shows the trend of Scale-RAE. On SeFi-Image diversity and
    FID barely change with $\tau$. The dotted line marks our $\tau = 0.02$.}
  \label{fig:keff_backbones}
\end{figure}


==> figures/keff_backbones/values.tex <==
\expandafter\def\csname divkeff@svg@lpips\endcsname{(1,-9.663) (1.521,-6.748) (5.228,-1.994) (15.06,0.767) (24.7,1.840) (46.65,2.607)}%
\expandafter\def\csname divkeff@svg@dreamsim\endcsname{(1,-7.440) (1.521,-2.976) (5.228,4.464) (15.06,10.119) (24.7,11.905) (46.65,13.988)}%
\expandafter\def\csname divkeff@svg@vendi\endcsname{(1,-2.139) (1.521,0.000) (5.228,4.614) (15.06,7.676) (24.7,8.809) (46.65,10.151)}%
\expandafter\def\csname divkeff@svg@fid\endcsname{(1,-24.484) (1.521,-24.305) (5.228,-24.126) (15.06,-23.946) (24.7,-21.928) (46.65,-20.942)}%
\expandafter\def\csname divkeff@sefi@lpips\endcsname{(1,0.923) (1.521,1.231) (15.06,1.846) (24.7,2.000) (46.65,2.154)}%
\expandafter\def\csname divkeff@sefi@dreamsim\endcsname{(1,16.099) (1.521,16.409) (15.06,18.266) (24.7,18.576) (46.65,19.505)}%
\expandafter\def\csname divkeff@sefi@vendi\endcsname{(1,14.298) (1.521,14.431) (15.06,15.361) (24.7,15.626) (46.65,15.981)}%
\expandafter\def\csname divkeff@sefi@fid\endcsname{(1,-16.077) (1.521,-15.675) (15.06,-15.327) (24.7,-15.380) (46.65,-15.005)}%
\expandafter\def\csname divkeff@xdef\endcsname{15.06}%
\expandafter\def\csname divkeff@xstat\endcsname{mean}%


==> figures/keff_hist/fig_keff_hist.tex <==
\begin{figure}[b]%
  \centering
  \includegraphics[width=\linewidth]{figures/keff_hist/keff_hist.pdf}
  \caption{\textbf{Effective number of neighbours.} Share of the $5{,}000$ prompts by
  $k_\mathrm{eff} = 1 / \sum_j \alpha_j^2$ at $k = 50$. Ours, $\tau = 0.02$, is in bold.
  Bars above $20\%$ are cut and labelled with their height.}
  \label{fig:keff_hist}
\end{figure}


==> figures/pareto/fig_pareto.tex <==
\begin{figure}[t]
  \centering
  \input{figures/pareto/values}%
  \newcommand{\ptw}{0.80\linewidth}%
  \newcommand{\pth}{0.40\linewidth}%
  \newcommand{\ptfont}{\scriptsize}%
  \definecolor{ptbase}{HTML}{EB6834}%
  \definecolor{ptours}{HTML}{2A78D6}%
  \pgfplotsset{ptaxis/.style={width=\ptw, height=\pth, scale only axis, clip=false,
      axis x line*=bottom, axis y line*=left, grid=major, grid style={black!10, line width=0.3pt},
      tick label style={font=\ptfont}, label style={font=\ptfont},
      x tick label style={/pgf/number format/.cd, fixed, fixed zerofill, precision=2},
      major tick length=2pt, tick style={black!60, line width=0.4pt}, axis line style={black!70, line width=0.4pt},
      xlabel={CLIP $\uparrow$}, ylabel={FID-5k $\downarrow$}, xlabel style={yshift=3pt}, ylabel style={yshift=-3pt},
      title style={font=\small, yshift=-3pt}, enlarge x limits=0.07, enlarge y limits=0.13},
    ptline/.style={line width=1pt, mark options={solid, fill=#1, draw=white, line width=0.35pt}},
    pt base/.style={ptbase, ptline=ptbase, mark=triangle*, mark size=2.2pt},
    pt rsd/.style={ptours, ptline=ptours, mark=*, mark size=1.8pt}}%
  \tikzset{pt lab base/.style={font=\ptfont, text=ptbase, inner sep=1.5pt},
    pt lab rsd/.style={font=\ptfont, text=ptours, inner sep=1.5pt}}%
  \newcommand{\ptpanel}[4]{%
    \begin{tikzpicture}
      \begin{axis}[ptaxis, title={#1}, #4]
        #2
        #3
      \end{axis}
    \end{tikzpicture}}%
  \ifdefined\figcachebegin\figcachebegin{pareto}\fi
  \ptpanel{\paretoraename}{\paretoraebase}{\paretoraersd}{legend pos=north west, legend cell align=left,
    legend style={draw=none, fill=white, font=\ptfont, inner sep=1pt, nodes={inner sep=1pt}},
    legend entries={Released sampler ($50$ steps), \method{} ($8$ steps)}}\\[3pt]
  \ptpanel{\paretosvgname}{\paretosvgbase}{\paretosvgrsd}{}
  \ifdefined\figcacheend\figcacheend\fi
  \caption{\textbf{FID against alignment} over the guidance sweep of \cref{tab:guidance}. Each marker is one guidance scale, labeled with its $w$.}
  \label{fig:pareto}
\end{figure}


==> figures/pareto/values.tex <==
\newcommand{\paretoraebase}{%
  \addplot[pt base] coordinates {(0.4182,29.513) (0.4392,32.009) (0.4478,32.529) (0.4492,31.721) (0.4474,31.25)};
  \node[pt lab base, anchor=south east] at (axis cs:0.4182,29.513) {$w{=}1$};
  \node[pt lab base, anchor=south east] at (axis cs:0.4392,32.009) {2};
  \node[pt lab base, anchor=south] at (axis cs:0.4478,32.529) {4};
  \node[pt lab base, anchor=west] at (axis cs:0.4492,31.721) {6};
  \node[pt lab base, anchor=north] at (axis cs:0.4474,31.25) {8};}%
\newcommand{\paretoraersd}{%
  \addplot[pt rsd] coordinates {(0.3928,23.463) (0.4093,21.65) (0.4204,21.061) (0.4231,21.366) (0.421,23.361)};
  \node[pt lab rsd, anchor=north] at (axis cs:0.3928,23.463) {$w{=}1$};
  \node[pt lab rsd, anchor=north] at (axis cs:0.4093,21.65) {2};
  \node[pt lab rsd, anchor=north] at (axis cs:0.4204,21.061) {4};
  \node[pt lab rsd, anchor=west] at (axis cs:0.4231,21.366) {6};
  \node[pt lab rsd, anchor=south west] at (axis cs:0.421,23.361) {8};}%
\newcommand{\paretosvgbase}{%
  \addplot[pt base] coordinates {(0.3694,23.046) (0.4198,20.548) (0.4396,22.301) (0.4452,23.306) (0.4474,23.73)};
  \node[pt lab base, anchor=south] at (axis cs:0.3694,23.046) {$w{=}1$};
  \node[pt lab base, anchor=north] at (axis cs:0.4198,20.548) {2};
  \node[pt lab base, anchor=north west] at (axis cs:0.4396,22.301) {4};
  \node[pt lab base, anchor=north west] at (axis cs:0.4452,23.306) {6};
  \node[pt lab base, anchor=south east] at (axis cs:0.4474,23.73) {8};}%
\newcommand{\paretosvgrsd}{%
  \addplot[pt rsd] coordinates {(0.3895,16.218) (0.4121,16.041) (0.4304,16.962) (0.4377,17.877) (0.4411,18.556)};
  \node[pt lab rsd, anchor=north] at (axis cs:0.3895,16.218) {$w{=}1$};
  \node[pt lab rsd, anchor=north] at (axis cs:0.4121,16.041) {2};
  \node[pt lab rsd, anchor=north west] at (axis cs:0.4304,16.962) {4};
  \node[pt lab rsd, anchor=north west] at (axis cs:0.4377,17.877) {6};
  \node[pt lab rsd, anchor=south east] at (axis cs:0.4411,18.556) {8};}%
\newcommand{\paretoraename}{Scale-RAE}
\newcommand{\paretosvgname}{SVG-T2I}


==> figures/sefi1024_qual/fig_sefi1024_qual.tex <==
\input{figures/sefi1024_qual/values}
\begin{figure*}[t]
  \centering
  \definecolor{sqbase}{HTML}{EB6834}%
  \definecolor{sqrmg}{HTML}{4E9F5B}%
  \newcommand{\sqpanelw}{0.17}%
  \newcommand{\sqlabw}{0.045}%
  \newcommand{\sqcolsep}{1.5pt}%
  \newcommand{\sqpromptsep}{2.5pt}%
  \newcommand{\sqrowsep}{3pt}%
  \newcommand{\sqpromptfont}{\scriptsize}%
  \newcommand{\sqframe}{0.3pt}%
  \newcommand{\sqlabfont}{\footnotesize}%
  \newcommand{\sqbadgefont}{\scriptsize\bfseries}%
  \newcommand{\sqbadgesep}{3pt}%
  \setlength{\tabcolsep}{\sqcolsep}%
  \renewcommand{\arraystretch}{0}%
  \setlength{\fboxsep}{0pt}\setlength{\fboxrule}{\sqframe}%
  \newcommand{\sqv}[1]{\csname sefiqual@#1\endcsname}%
  \newcommand{\sqimg}[2]{\fbox{\includegraphics[width=\dimexpr\sqpanelw\linewidth-2\fboxrule\relax]{figures/sefi1024_qual/#1/#2.jpg}}}%
  \newcommand{\sqprompt}[1]{\parbox[b]{\sqpanelw\linewidth}{\centering\sqpromptfont\gridprompt{\sqv{#1}}}}%
  \ifdefined\sqph\else\newlength{\sqph}\fi\setlength{\sqph}{\sqpanelw\linewidth}%
  \newcommand{\sqlab}[2]{\parbox[b][\sqph][c]{\sqlabw\linewidth}{\centering\rotatebox{90}{\parbox{\sqph}{\centering\color{#1}#2}}}}%
  \newcommand{\sqbadge}[2]{\tikz[baseline=(t.base)]\node[fill=#1, text=white, rounded corners=2pt,
    inner xsep=2.5pt, inner ysep=1.6pt, font=\sqbadgefont] (t) {\sqv{#2}$\times$ faster};}%
  \newcommand{\sqrow}[1]{\sqimg{p03478}{#1} & \sqimg{p01251}{#1} & \sqimg{p03606}{#1} &
    \sqimg{p02271}{#1} & \sqimg{p04529}{#1}}%
  \ifdefined\tikzexternaldisable\tikzexternaldisable\fi
  \begin{tabular}{@{}cccccc@{}}
    & \sqprompt{p03478} & \sqprompt{p01251} & \sqprompt{p03606} &
    \sqprompt{p02271} & \sqprompt{p04529} \\[\sqpromptsep]
    \sqlab{sqbase}{\sqlabfont SeFi-Image} & \sqrow{base} \\[\sqrowsep]
    \sqlab{sqrmg}{\sqlabfont RMG\\[\sqbadgesep]\sqbadge{sqrmg}{ratiormg}} & \sqrow{rmg} \\[\sqrowsep]
    \sqlab{otherblue}{\sqlabfont\textbf{\method{} (ours)}\\[\sqbadgesep]\sqbadge{otherblue}{ratio}} & \sqrow{ours} \\
  \end{tabular}
  \ifdefined\tikzexternalenable\tikzexternalenable\fi
  \caption{\textbf{SeFi-Image at $1024$ pixels on COCO.} The released sampler with \sqv{base} steps
    (top), RMG with \sqv{rmg} (middle) and \method with \sqv{ours} (bottom), from the same noise.}
  \label{fig:sefi1024_qual}
\end{figure*}


==> figures/sefi1024_qual/values.tex <==
\expandafter\def\csname sefiqual@base\endcsname{50}%
\expandafter\def\csname sefiqual@rmg\endcsname{20}%
\expandafter\def\csname sefiqual@ours\endcsname{8}%
\expandafter\def\csname sefiqual@ratio\endcsname{6.25}%
\expandafter\def\csname sefiqual@ratiormg\endcsname{2.5}%
\expandafter\def\csname sefiqual@p03478\endcsname{Cattle lie in the grass to chew their cud.}%
\expandafter\def\csname sefiqual@p01251\endcsname{A woman walking while carrying bananas on her hat.}%
\expandafter\def\csname sefiqual@p03606\endcsname{A woman is carrying many packages in an office building}%
\expandafter\def\csname sefiqual@p04544\endcsname{A female is talking on the phone and a laptop on a table}%
\expandafter\def\csname sefiqual@p02271\endcsname{The man is trying to hit the baseball during the game.}%
\expandafter\def\csname sefiqual@p04529\endcsname{A man in black carrying a sheep on his shoulders.}%


==> figures/supp_qual/fig_supp_qual_art_anime.tex <==
\input{figures/supp_qual/values}%
\begin{figure*}[p]%
  \begin{minipage}[t][0.995\textheight][s]{\textwidth}
  \centering
  \input{figures/supp_qual/layout}%
  \qheadrow
  \qrow{art}{rae}{Scale-RAE}
  \qrow{art}{sefi}{SeFi-Image}
  \qrow{art}{svg}{SVG-T2I}
  \vspace{-\dimexpr\qrowsep+\qcapup\relax}
  \caption{\textbf{Qualitative comparison on WikiArt.} As \cref{fig:supp_qual_coco}, on WikiArt prompts with the WikiArt corpus.}
  \label{fig:supp_qual_art}
  \vspace{\qfigsep}\vfill%
  \qrow{anime}{rae}{Scale-RAE}
  \qrow{anime}{sefi}{SeFi-Image}
  \qrow{anime}{svg}{SVG-T2I}
  \vspace{-\dimexpr\qrowsep+\qcapup\relax}
  \caption{\textbf{Qualitative comparison on Anime.} As \cref{fig:supp_qual_coco}, on Anime prompts with the Anime corpus. Long prompts are shortened to their first sentence.}
  \label{fig:supp_qual_anime}
  \end{minipage}
\end{figure*}


==> figures/supp_qual/fig_supp_qual_coco.tex <==
\input{figures/supp_qual/values}%
\begin{figure*}[t]
  \centering
  \input{figures/supp_qual/layout}%
  \qheadrow
  \qrow{coco}{rae}{Scale-RAE}
  \qrow{coco}{sefi}{SeFi-Image}
  \qrow{coco}{svg}{SVG-T2I}
  \vspace{-\dimexpr\qrowsep+\qcapup\relax}
  \caption{\textbf{Qualitative comparison on COCO.} The released sampler with $50$ steps, RMG with $20$ and \method with $8$, from the same noise, on each backbone.}
  \label{fig:supp_qual_coco}
\end{figure*}


==> figures/supp_qual/layout.tex <==
\newcommand{\qpanelw}{0.154}%
\newcommand{\qcolsep}{1.5pt}%
\newcommand{\qlabw}{10pt}%
\newcommand{\qpromptsep}{1pt}%
\newcommand{\qrowsep}{2pt}%
\newcommand{\qheadsep}{1pt}%
\newcommand{\qcapup}{3pt}%
\newcommand{\qfigsep}{6pt}%
\newcommand{\qpromptfont}{\scriptsize}%
\newcommand{\qheadfont}{\footnotesize}%
\newcommand{\qlabfont}{\footnotesize}%
\newcommand{\qframe}{0.3pt}%
\definecolor{qbase}{HTML}{EB6834}%
\definecolor{qrmg}{HTML}{4E9F5B}%
\setlength{\fboxsep}{0pt}\setlength{\fboxrule}{\qframe}%
\ifdefined\qtripw\else\newlength{\qtripw}\newlength{\qpw}\fi
\setlength{\qpw}{\qpanelw\linewidth}%
\setlength{\qtripw}{3\qpw}\addtolength{\qtripw}{\qcolsep}\addtolength{\qtripw}{\qcolsep}%
\newcommand{\qv}[1]{\csname suppqual@#1\endcsname}%
\newcommand{\qimg}[2]{\fbox{\includegraphics[width=\dimexpr\qpw-2\fboxrule\relax]{figures/supp_qual/#1/#2.jpg}}}%
\newcommand{\qnone}{\fbox{\parbox[b][\dimexpr\qpw-2\fboxrule\relax][c]{\dimexpr\qpw-2\fboxrule\relax}{\centering\tiny pending}}}%
\newcommand{\qtrip}[3]{\begin{minipage}[b]{\qtripw}\centering
    {\qpromptfont\gridprompt{\qv{#1@#2@#3}}\par}\vspace{\qpromptsep}%
    \ifcsname suppqual@#1@#2@#3@idx\endcsname
      \qimg{#1/#2/\qv{#1@#2@#3@idx}}{base}\hspace{\qcolsep}\qimg{#1/#2/\qv{#1@#2@#3@idx}}{rmg}\hspace{\qcolsep}%
      \qimg{#1/#2/\qv{#1@#2@#3@idx}}{ours}%
    \else\qnone\hspace{\qcolsep}\qnone\hspace{\qcolsep}\qnone\fi
  \end{minipage}}%
\newcommand{\qhead}{\begin{minipage}[b]{\qtripw}\qheadfont
    \parbox[b]{\qpw}{\centering\color{qbase}Baseline}\hspace{\qcolsep}%
    \parbox[b]{\qpw}{\centering\color{qrmg}RMG}\hspace{\qcolsep}%
    \parbox[b]{\qpw}{\centering\color{otherblue}\textbf{\method{} (ours)}}%
  \end{minipage}}%
\newcommand{\qlab}[1]{\parbox[b][\qpw][c]{\qlabw}{\centering\rotatebox{90}{\qlabfont #1}}}%
\newcommand{\qrow}[3]{\noindent\qlab{#3}\hfill\qtrip{#1}{#2}{1}\hfill\qtrip{#1}{#2}{2}\par\vspace{\qrowsep}}%
\newcommand{\qheadrow}{\noindent\hspace*{\qlabw}\hfill\qhead\hfill\qhead\par\vspace{\qheadsep}}%


==> figures/supp_qual/values.tex <==
\expandafter\def\csname suppqual@coco@rae@1\endcsname{A red fire hydrant sitting on the side of a road.}%
\expandafter\def\csname suppqual@coco@rae@1@idx\endcsname{p03797}%
\expandafter\def\csname suppqual@coco@rae@2\endcsname{A red and white boat floating along a river.}%
\expandafter\def\csname suppqual@coco@rae@2@idx\endcsname{p02854}%
\expandafter\def\csname suppqual@coco@svg@1\endcsname{A large white clock tower filled with light.}%
\expandafter\def\csname suppqual@coco@svg@1@idx\endcsname{p02552}%
\expandafter\def\csname suppqual@coco@svg@2\endcsname{An elaborate church with tiled floors and stained glass.}%
\expandafter\def\csname suppqual@coco@svg@2@idx\endcsname{p04081}%
\expandafter\def\csname suppqual@coco@sefi@1\endcsname{three dogs on a field of green grass}%
\expandafter\def\csname suppqual@coco@sefi@1@idx\endcsname{p02322}%
\expandafter\def\csname suppqual@coco@sefi@2\endcsname{A man in a suit is wearing a lit up tie.}%
\expandafter\def\csname suppqual@coco@sefi@2@idx\endcsname{p00207}%
\expandafter\def\csname suppqual@anime@rae@1\endcsname{A portrait of a young woman with short, layered blue hair and large blue eyes, wearing a white dress with a blue sash tied at the waist.}%
\expandafter\def\csname suppqual@anime@rae@1@idx\endcsname{p03577}%
\expandafter\def\csname suppqual@anime@rae@2\endcsname{A close-up portrait of a young girl with long, straight white hair, large blue eyes, and a small red hair accessory.}%
\expandafter\def\csname suppqual@anime@rae@2@idx\endcsname{p04964}%
\expandafter\def\csname suppqual@anime@svg@1\endcsname{A close-up portrait of a young girl with bright blonde hair styled in pigtails and large, bright blue eyes.}%
\expandafter\def\csname suppqual@anime@svg@1@idx\endcsname{p03557}%
\expandafter\def\csname suppqual@anime@svg@2\endcsname{A young man with blonde hair, wearing a brown jacket and jeans, sits on the railing of a rooftop overlooking a cityscape during a dramatic sunset.}%
\expandafter\def\csname suppqual@anime@svg@2@idx\endcsname{p04327}%
\expandafter\def\csname suppqual@anime@sefi@1\endcsname{A close-up of a young woman with long, light purple hair, wearing a horned headpiece and a futuristic, metallic headband.}%
\expandafter\def\csname suppqual@anime@sefi@1@idx\endcsname{p02706}%
\expandafter\def\csname suppqual@anime@sefi@2\endcsname{A young woman with large, pointed ears and light brown hair, wearing a purple dress, a dark vest, and metallic arm and leg armor.}%
\expandafter\def\csname suppqual@anime@sefi@2@idx\endcsname{p03217}%
\expandafter\def\csname suppqual@art@rae@1\endcsname{A painting of a cliff overlooking the ocean, with a small boat in the distance and a cloudy sky above.}%
\expandafter\def\csname suppqual@art@rae@1@idx\endcsname{p03656}%
\expandafter\def\csname suppqual@art@rae@2\endcsname{A black and white sketch of trees and bushes, rendered in an impressionistic style.}%
\expandafter\def\csname suppqual@art@rae@2@idx\endcsname{p04640}%
\expandafter\def\csname suppqual@art@svg@1\endcsname{A painting of a mountain view with a vase of white flowers in the foreground.}%
\expandafter\def\csname suppqual@art@svg@1@idx\endcsname{p01685}%
\expandafter\def\csname suppqual@art@svg@2\endcsname{A cowboy sits on a rock, gazing up at the night sky.}%
\expandafter\def\csname suppqual@art@svg@2@idx\endcsname{p00216}%
\expandafter\def\csname suppqual@art@sefi@1\endcsname{A painting of a bird and a lion with a dark background.}%
\expandafter\def\csname suppqual@art@sefi@1@idx\endcsname{p01937}%
\expandafter\def\csname suppqual@art@sefi@2\endcsname{A painting of three children on a beach, with one child in a white dress and two in white dresses, holding hands and walking towards the water.}%
\expandafter\def\csname suppqual@art@sefi@2@idx\endcsname{p04867}%


==> figures/svg1024_qual/fig_svg1024_qual.tex <==
\input{figures/svg1024_qual/values}
\begin{figure*}[t]
  \centering
  \definecolor{sqbase}{HTML}{EB6834}%
  \definecolor{sqrmg}{HTML}{4E9F5B}%
  \newcommand{\sqpanelw}{0.17}%
  \newcommand{\sqlabw}{0.045}%
  \newcommand{\sqcolsep}{1.5pt}%
  \newcommand{\sqpromptsep}{2.5pt}%
  \newcommand{\sqrowsep}{3pt}%
  \newcommand{\sqpromptfont}{\scriptsize}%
  \newcommand{\sqframe}{0.3pt}%
  \newcommand{\sqlabfont}{\footnotesize}%
  \newcommand{\sqbadgefont}{\scriptsize\bfseries}%
  \newcommand{\sqbadgesep}{3pt}%
  \setlength{\tabcolsep}{\sqcolsep}%
  \renewcommand{\arraystretch}{0}%
  \setlength{\fboxsep}{0pt}\setlength{\fboxrule}{\sqframe}%
  \newcommand{\sqv}[1]{\csname svgqual@#1\endcsname}%
  \newcommand{\sqimg}[2]{\fbox{\includegraphics[width=\dimexpr\sqpanelw\linewidth-2\fboxrule\relax]{figures/svg1024_qual/#1/#2.jpg}}}%
  \newcommand{\sqprompt}[1]{\parbox[b]{\sqpanelw\linewidth}{\centering\sqpromptfont\gridprompt{\sqv{#1}}}}%
  \ifdefined\sqph\else\newlength{\sqph}\fi\setlength{\sqph}{\sqpanelw\linewidth}%
  \newcommand{\sqlab}[2]{\parbox[b][\sqph][c]{\sqlabw\linewidth}{\centering\rotatebox{90}{\parbox{\sqph}{\centering\color{#1}#2}}}}%
  \newcommand{\sqbadge}[2]{\tikz[baseline=(t.base)]\node[fill=#1, text=white, rounded corners=2pt,
    inner xsep=2.5pt, inner ysep=1.6pt, font=\sqbadgefont] (t) {\sqv{#2}$\times$ faster};}%
  \newcommand{\sqrow}[1]{\sqimg{p03273}{#1} & \sqimg{p03876}{#1} & \sqimg{p01033}{#1} &
    \sqimg{p02913}{#1} & \sqimg{p02442}{#1}}%
  \ifdefined\tikzexternaldisable\tikzexternaldisable\fi
  \begin{tabular}{@{}cccccc@{}}
    & \sqprompt{p03273} & \sqprompt{p03876} & \sqprompt{p01033} &
    \sqprompt{p02913} & \sqprompt{p02442} \\[\sqpromptsep]
    \sqlab{sqbase}{\sqlabfont SVG-T2I} & \sqrow{base} \\[\sqrowsep]
    \sqlab{sqrmg}{\sqlabfont RMG\\[\sqbadgesep]\sqbadge{sqrmg}{ratiormg}} & \sqrow{rmg} \\[\sqrowsep]
    \sqlab{otherblue}{\sqlabfont\textbf{\method{} (ours)}\\[\sqbadgesep]\sqbadge{otherblue}{ratio}} & \sqrow{ours} \\
  \end{tabular}
  \ifdefined\tikzexternalenable\tikzexternalenable\fi
  \caption{\textbf{SVG-T2I at its released $1024$ pixels on COCO.} The released sampler with \sqv{base} steps
    (top), RMG with \sqv{rmg} (middle) and \method with \sqv{ours} (bottom), from the same noise.}
  \label{fig:svg1024_qual}
\end{figure*}


==> figures/svg1024_qual/values.tex <==
\expandafter\def\csname svgqual@base\endcsname{50}%
\expandafter\def\csname svgqual@rmg\endcsname{20}%
\expandafter\def\csname svgqual@ours\endcsname{8}%
\expandafter\def\csname svgqual@ratio\endcsname{6.25}%
\expandafter\def\csname svgqual@ratiormg\endcsname{2.5}%
\expandafter\def\csname svgqual@w\endcsname{6}%
\expandafter\def\csname svgqual@p03273\endcsname{A dog is tied to a fire hydrant.}%
\expandafter\def\csname svgqual@p03876\endcsname{Small bedroom with a bed and dresser with a small monitor on top of it.}%
\expandafter\def\csname svgqual@p01033\endcsname{A large black semi parked in a parking lot.}%
\expandafter\def\csname svgqual@p02913\endcsname{Several different fire hydrants that have been painted various colors.}%
\expandafter\def\csname svgqual@p03329\endcsname{A white and red plane parked on a tarmac}%
\expandafter\def\csname svgqual@p02442\endcsname{A microwave sitting on top of a wooden shelf.}%


==> figures/t0_line/fig_t0_line.tex <==
\begin{figure*}[t]
  \centering
  \input{figures/t0_line/values}%
  \newcommand{\tlw}{0.86\linewidth}%
  \newcommand{\tlh}{0.15\linewidth}%
  \newcommand{\tlgap}{2pt}%
  \newcommand{\tlvgap}{3pt}%
  \newcommand{\tlfont}{\footnotesize}%
  \newcommand{\tlnotefont}{\scriptsize}%
  \newcommand{\tlpromptsep}{3pt}%
  \newcommand{\tlpromptfont}{\footnotesize}%
  \definecolor{tlfid}{HTML}{2A78D6}%
  \definecolor{tlmem}{HTML}{C0392B}%
  \pgfmathsetlengthmacro\tltile{\tlw/\tln-\tlgap}%
  \pgfmathsetmacro\tlxmax{\tln-0.5}%
  \pgfmathtruncatemacro\tllast{\tln-1}%
  \pgfplotsset{tlaxis/.style={width=\tlw, height=\tlh, scale only axis, xmin=-0.5, xmax=\tlxmax,
      xtick={0,...,\tllast}, clip=false, tick label style={font=\tlfont}, label style={font=\tlfont},
      major tick length=2pt, tick style={black!60, line width=0.4pt}}}%
  \ifdefined\figcachebegin\figcachebegin{t0_line}\fi
  \begin{tikzpicture}
    \begin{axis}[tlaxis, name=fid, axis x line*=bottom, axis y line*=left,
        ymin=10, ymax=23.5, ytick={12,16,20}, ymajorgrids, grid style={black!12, line width=0.3pt},
        xticklabels/.expand once=\tlxticks, xlabel={$t_0$}, xlabel style={yshift=3pt},
        ylabel={FID-5k $\downarrow$}, ylabel style={text=tlfid, yshift=-3pt}]
      \fill[black!6] (axis cs:1.5,10) rectangle (axis cs:2.5,23.5);
      \edef\tlplot{\noexpand\addplot[tlfid, line width=1pt, mark=*, mark size=1.5pt] coordinates {\tlfid};}\tlplot
    \end{axis}
    \begin{axis}[tlaxis, axis x line=none, axis y line*=right, ymode=log, ymin=0.005, ymax=20,
        ytick={0.01,0.1,1,10}, yticklabels={$0.01$,$0.1$,$1$,$10$}, yminorticks=false,
        ylabel={Near-dup.\ (\%) $\downarrow$}, ylabel style={text=tlmem, yshift=3pt}]
      \draw[tlmem, line width=0.6pt, dash pattern=on 3pt off 2pt] (axis cs:-0.5,\tlmembase) -- (axis cs:\tlxmax,\tlmembase);
      \node[font=\tlnotefont, text=tlmem, anchor=south, inner sep=1pt] at (axis cs:0.5,\tlmembase) {baseline};
      \edef\tlplot{\noexpand\addplot[tlmem, line width=1pt, mark=square*, mark size=1.4pt] coordinates {\tlmem};}\tlplot
    \end{axis}
    \foreach \f [count=\i from 0] in \tltiles
      \node[anchor=south, inner sep=0pt] (tile\i) at ($(fid.north west)!{(\i+0.5)/\tln}!(fid.north east)+(0,\tlvgap)$)
        {\includegraphics[width=\tltile]{figures/t0_line/\f.jpg}};
    \node[inner sep=0pt, anchor=south, font=\tlpromptfont, text width=\tlw, align=center]
      at ($(tile0.north west)!0.5!(tile\tllast.north east)+(0,\tlpromptsep)$) {\gridprompt{\tlprompt}};
  \end{tikzpicture}
  \ifdefined\figcacheend\figcacheend\fi
  \caption{\textbf{Noise level against memorization.} Above: one SVG-T2I prompt and noise draw at each
    $t_0$ ($t_0 = 0$ is the released sampler at its 50 steps). Below:
    the FID-5k and near-duplicate rate. FID keeps falling past $t_0 = 0.05$, but from $t_0 = 0.1$
    the near-duplicate rate rises above the baseline's (dashed).}
  \label{fig:t0_line}
\end{figure*}


==> figures/t0_line/values.tex <==
\def\tlfid{(0,22.3) (1,21.08) (2,16.96) (3,15.44) (4,15.29)}%
\def\tlmem{(0,0.04) (1,0.02) (2,0.02) (3,0.48) (4,9.84)}%
\def\tlmembase{0.04}%
\def\tlxticks{$0$,$0.02$,$0.05$,$0.1$,$0.2$}%
\def\tln{5}%
\def\tltiles{p02218/t000,p02218/t002,p02218/t005,p02218/t010,p02218/t020}%
\def\tlprompt{A yellow BMW touring motorcycle parked in the street as people look on from behind a steel rail on the sidewalk.}%


==> sections/app/A_additional.tex <==
\section{Additional results}
\label{app:results}
\subsection{Store sizes and latency}
\label{app:cost}
\paragraph{Store sizes.}
\Cref{tab:store_size} gives the exact size of every store. The fp16 latents of each corpus in each
backbone's latent space, of which a prompt reads $k$ rows, and the SigLIP-2 keys which the search
reads in full and which all three backbones share.

\paragraph{Latency.}
\Cref{tab:latency} times one prompt at batch size $1$ on one GPU, as the median over $100$ prompts for
the read and over $20$ for sampling ($10$ on SeFi-Image). The one-time read includes the SigLIP-2 embedding of the prompt,
the exact search over the shared keys and the read of the
$k = 50$ latents of \method or the $20$ of RMG's bank, done once per prompt. It takes $2$ to $7$\,ms,
against $32$ to $37$\,ms for one forward pass of Scale-RAE or SVG-T2I.
Sampling time is the wall-clock time to generate one image without the backbone's text encoder and decoder,
which every sampler runs once per image. It covers the denoising steps and for RMG and \method the one-time read too.
On Scale-RAE, a guided step of \method and RMG
runs its two passes one after the other. \method is $3.15\times$ faster than the released sampler on
Scale-RAE, close to its $3.125\times$ fewer network evaluations, and
$6.24\times$ and $6.23\times$ faster on SVG-T2I and SeFi-Image, close to its $6.25\times$ fewer
steps. RMG, with $20$ guided steps, is $1.23\times$, $2.50\times$ and $2.51\times$ faster than the
released sampler, so \method is $2.5$ to $2.6\times$ faster than RMG on all three.
SeFi-Image's text encoder and decoder are not timed separately, so we take its step as the
time difference between $50$ and $8$ steps of its released sampler divided by $42$.

\subsection{Equal step counts}
\label{app:prdc}
\Cref{tab:main} compares methods at their default settings. Here
Gaussian sampling, RMG and \method run at the same number of steps, from $4$ to $50$, on COCO
(\cref{fig:fid_vs_nfe,tab:app_prdc}).

\method has a lower FID than Gaussian sampling at every step count on all three backbones, so its
gain does not come from taking fewer steps. More steps change little for either. From $8$ to $50$
steps Gaussian sampling gains at most $1.4$ FID and \method moves by at most $1.3$, so comparing
against the released samplers at $50$ steps does not handicap them. The exception is SeFi-Image
which is $2.0$ points better at its $8$ steps point and there \method at $8$ steps still beats it, $31.60$ against
$35.32$.
On Scale-RAE the released sampler is unguided ($w=1$), so at the same step count
\method makes twice its network evaluations. Guidance does not help the released sampler, whose FID
at $w = 4$ and $50$ steps rises to $32.53$ (\cref{tab:guidance}).
\input{tables/store_size/tab_store_size}
\input{tables/latency/tab_latency}
\input{tables/app_prdc/app_prdc}
\input{figures/fid_vs_nfe/fid_vs_nfe}

One might wonder if \method buys its FID by dropping modes, which would lower recall and coverage but it does not.
Both are higher than Gaussian sampling's at every step count on all three backbones. Precision and density
are higher at every step count on SVG-T2I, and on Scale-RAE and SeFi-Image they are either higher or
within $0.025$ of Gaussian sampling's.
\newpage

\subsection{Another solver}
\label{app:solver}
\Cref{tab:solver} repeats the comparison at $N = 8$ with DPM-Solver++(2M)~\cite{lu2022dpmsolverpp}, a
second-order multistep solver that makes one network call per step on the same time grid.
It lowers FID by $0.2$ to $0.8$ for both Gaussian sampling and \method, and \method's gain over Gaussian sampling
barely changes - $9.2$ and $9.1$ FID points on Scale-RAE with Euler and DPM-Solver++, $6.8$ and $6.5$
on SVG-T2I, and $3.7$ and $3.9$ on SeFi-Image.
\input{tables/solver/tab_solver}

\subsection{Memorisation audit}
\label{app:memorization}
\input{figures/t0_line/fig_t0_line}
\input{tables/memorization/memorization}
\input{tables/fd_cmmd/fd_cmmd}

An anchor drawn from real images invites the question of whether the output is one of the retrieved images~\cite{carlini2023extracting,somepalli2023diffusion}.
Copying would pay off in FID. Decoding the nearest retrieved latent with no generation at all
scores $14.03$ on Scale-RAE and $14.35$ on SVG-T2I. We
score the maximum similarity of every generation to the whole corpus with SSCD~\cite{pizzi2022self}
and read it against the real held-out image
belonging to each prompt, scored the same way. \vadjust{\vfill\penalty-10000\null\vfill\penalty-10000}%
SSCD is an image descriptor trained for copy detection, so an image and its edited copies (cropped, recoloured, overlaid) get close descriptors and two images are compared by their cosine similarity.

The Held-out images are the informative part of \cref{tab:memorization}. Held-out images exceed the
conventional copy threshold of $0.5$~\cite{somepalli2023diffusion} for $3.82$ to $6.00\%$ of
prompts, because real images of the same subject resemble each other. \method stays at or below
$0.32\%$ in all nine settings and at most $0.16$ points above
the released sampler's. RMG reaches $1.10\%$ on Scale-RAE on Anime. Moving the start further along the
path raises the rate above the released sampler's from $t_0 = 0.1$ (\cref{fig:t0_line}).

\subsection{\texorpdfstring{FD$_\text{DINOv2}$}{FD-DINOv2} and CMMD}
\label{app:fd_cmmd}
\input{tables/rmg_k20/tab_rmg_k20}
FID and KID compare Inception features, which can disagree with human judgement on modern
generators~\cite{stein2023exposing,jayasumana2024rethinking}. \Cref{tab:fd_cmmd} repeats the comparison
of \cref{tab:main} in two other feature spaces, against the same held-out images.
FD$_\text{DINOv2}$~\cite{stein2023exposing} is the Fr\'echet distance between DINOv2 ViT-L/14 features,
and CMMD~\cite{jayasumana2024rethinking} is the maximum mean discrepancy between CLIP ViT-L/14
embeddings under a Gaussian kernel of bandwidth $10$, reported $\times 10^3$ as in its reference
implementation. \method has the lowest FD$_\text{DINOv2}$ in all nine settings and the lowest CMMD in
eight. The exception is SeFi-Image on COCO, where the released sampler and RMG reach a lower CMMD,
$0.559$ and $0.579$ against $0.602$. SeFi-Image generates in a space built on DINOv2 features, where its anchor is also computed,
so on SeFi-Image CMMD is the more independent of the two.

\subsection{RMG at the same \texorpdfstring{$k$}{k}}
\label{app:rmg}
\Cref{tab:main} gives \method $k = 50$ neighbours and RMG a bank of $20$, the bank size of their
paper. \Cref{tab:app_rmg} removes that difference and lets both methods read the same $k$ images that our
search returns for each COCO val2017 prompt, at $k = 20$ and at $k = 50$. Each method is at its own number of
steps, $8$ for \method and $20$ for RMG.

At both values of $k$, \method has the lowest FID and KID on Scale-RAE and SVG-T2I and higher diversity than
RMG on almost all metrics, while RMG keeps the higher CLIP on Scale-RAE. On SeFi-Image the two are
almost level in FID and KID while RMG has slightly higher diversity and \method has slightly higher CLIP.
From $k = 20$ to $k = 50$ the FID of \method moves by at most $0.11$.

\subsection{Per-prompt diversity}
\label{app:diversity}
\Cref{fig:diversity_bars} shows the per-prompt diversity on COCO discussed in \cref{sec:exp:diversity},
\method and RMG at their default settings, each reported as the change from its backbone's released sampler. \Cref{fig:div_grid} shows four samples per prompt from each method.

\input{figures/diversity_bars/fig_diversity_bars}
\input{figures/div_grid/fig_div_grid}%


==> sections/app/B_implementation.tex <==
\section{Implementation details}
\label{app:setup}

\paragraph{Backbones.}
All three backbones are used exactly as released, with every weight frozen, and none is adapted to
\method in any way. Scale-RAE~\cite{tong2026scalerae} pairs a Qwen2.5-1.5B text encoder with a
$2.4$B-parameter LightningDiT velocity network that generates in the latent space of a
representation autoencoder over SigLIP-2 so400m/14~\cite{tschannen2025siglip2} at $224$ pixels, so
one latent is $256$ tokens of $1152$ channels, $D = 294{,}912$ values.
SVG-T2I~\cite{shi2025svgt2i,shi2025svg} pairs a Gemma-2-2B text encoder with a $2.6$B-parameter
Next-DiT over a semantic autoencoder on DINOv3 ViT-S/16+~\cite{simeoni2025dinov3} at $256$ pixels,
so one latent is $256$ tokens of $384$ channels, $D = 98{,}304$. These are the stage-1 checkpoints of
its progressive training, the NextDiT and the autoencoder at $256$ pixels, which we use because of our
compute budget. We show some examples of the default release, the stage-4 fine-tuned at $1024$ pixels in \cref{fig:svg1024_qual}.
SeFi-Image~\cite{feng2026sefi}, in its 2B base release, pairs a Qwen3-VL text encoder with a
transformer that generates two latents: a semantic one, DINOv2-L~\cite{oquab2023dinov2} patch
features compressed to $1024$ tokens of $16$ channels, and a texture one in the
FLUX.2~\cite{bfl2025flux2} VAE, decoded at $512$ pixels (examples at $1024$ in \cref{fig:sefi1024_qual}). No two share a component: text
encoder, velocity network, visual encoder, latent width and output resolution all differ.

\paragraph{Step schedules.}
Each backbone is integrated on its own released warp, subsampled as described in
\cref{sec:preliminaries}. Scale-RAE ships that warp as a thousand-point table produced by its own
sampler. SVG-T2I ships it in closed form as $t \mapsto t/(t + 6 - 6t)$. SeFi-Image ships a
shifted grid on which its semantic latent runs $0.1$ ahead of its texture latent. \method starts the
semantic latent at $t_0$ from the anchor and the texture latent from noise, a state the released
sampler itself passes through in its first phase, and then follows the released grid.

\paragraph{Retrieval.}
The index is built once, offline. On COCO, a corpus image's key is the mean of the SigLIP-2 text embeddings
of its five COCO captions~\cite{lin2014microsoft,chen2015cococaptions}, renormalised to the unit sphere, under the
so400m/14 text tower. On Anime and WikiArt it is the embedding of its one caption. A prompt is embedded by the same tower, so the search compares text to text
and never crosses the encoder's modality gap. On Scale-RAE this is the same SigLIP-2 checkpoint whose image tower defines the backbone's latent
space, so retrieval and generation share a model there. SVG-T2I and SeFi-Image share nothing with it,
and \method lowers FID on all three on COCO (\cref{tab:main}). The search itself is exact, one matrix product of the
query against the key matrix ($118{,}287 \times 1152$ on COCO) followed by a top-$k$. The $k$ latents are then
read from a memory-mapped fp16 array with one row per corpus image, so a prompt touches
$k$ rows and no more.

\paragraph{RMG.}
We implement RMG from the equations of \citet{curvo2026follow} as published. The guidance scale
$w = 3.5$, which the paper does not state, we take from their released code. At every step, with $\vv$ the guided velocity at
$\vz_t$, the model's estimate of the clean latent is $\hat\vz_1 = \vz_t + (1 - t)\, \vv$, the bank
estimate is
\begin{gather}
  \bar\vz = \sum_{j \in \gI_{k}(\vq)} \beta_j \vz_j, \label{eq:rmg} \\
  \beta = \softmax_{j \in \gI_{k}(\vq)} \bigg( -\frac{\norm{\vz_t - t \vz_j}^2}{2 \sqrt{D}\, (1 - t)^2} \bigg), \nonumber
\end{gather}
over the whole bank with no top-$k$ inside it, and the step uses
$\vv + \gamma_t (\bar\vz - \hat\vz_1) / (1 - t)$ with $\gamma_t = \gamma_0 (1 - t)^2$, and
$\gamma_t = 0$ for $t \geq 0.85$. Their time runs as ours, from noise at $t = 0$ to data at $t = 1$, so
the schedule needs no conversion. The bank is the $k = 20$ corpus latents that our search returns for
the prompt, the same latents \method averages into $\vmu$ at $k = 20$, and the nearest $20$ of its
$50$ in \cref{tab:main}, in the backbone's own latent units.
\citet{curvo2026follow} develop the method in the VAE latent space of FLUX.2-klein, where a latent
records appearance. Our backbones generate in semantic latent spaces, and nothing in the equations
above depends on which kind of space it is, so we apply them as they are. On SeFi-Image the correction
acts on the semantic latent only, where the anchor of \method also enters. Sampling uses a guidance
scale of $w = 3.5$ on each backbone's released step grid, at the $20$ steps of their evaluation protocol,
the setting \cref{tab:main} reports. We also run it from $4$ to $50$ steps on COCO (\cref{tab:app_prdc}).
The strength $\gamma_0$, which their paper sets per task
between $0.2$ and $1.0$, is the one free parameter: we try $\gamma_0 \in \{0.2, 0.5, 1.0\}$ on each
backbone and dataset and keep the value with the lowest KID.

\input{figures/svg1024_qual/fig_svg1024_qual}%

\paragraph{Anime and WikiArt.}
Both come from the Hugging Face Hub~\cite{noneyet2026animecaptions,atermors2026wikiartrecaption}, with one caption per image, and are filtered the same way, in
this order. A pair is dropped if its caption contains one of $28$ sexual terms (such as \emph{nude},
\emph{lingerie} or \emph{erotic}), if its caption exceeds the $64$ tokens of the SigLIP-2 text
encoder, so that no key or prompt is truncated, or if its image bytes or its caption repeat an earlier
pair. An image classifier for not-safe-for-work content (\texttt{Falconsai/nsfw\_image\_detection})
then removes every image it scores above $0.5$. Of the remaining pairs, $5{,}000$ are held out at
random, and every corpus image within SigLIP-2 image cosine similarity $0.95$ of a held-out
one is removed, so that no prompt can retrieve its own reference. Of the $337{,}038$ Anime pairs, these
steps remove $35{,}552$, $162{,}362$, $205$ and $11{,}585$, then $1{,}524$ near-copies, leaving a
corpus of $120{,}810$. Of the $81{,}355$ WikiArt pairs they remove $2{,}321$, $10$, $3{,}887$, $244$
and $372$, leaving $69{,}521$.

\paragraph{Metrics.}
FID~\cite{heusel2017gans} is FID-5k unless stated otherwise, computed with pytorch-fid's InceptionV3 against the $5{,}000$ held-out
images. Generations and reference images receive identical
preprocessing, shorter side resized and centre cropped to $224$ for Scale-RAE and to $256$ for every
other model, so the number does not measure a
resize artefact. With $5{,}000$ references the estimate is biased upward, so it is comparable
across our cells and not to FID-50k numbers reported elsewhere.
KID is the unbiased squared MMD between the same Inception features under the cubic polynomial
kernel of \citet{binkowski2018demystifying}, reported $\times 10^3$ as the mean over $100$ random
subsets of $1{,}000$ generations and $1{,}000$ references, their protocol. Its expected value does
not depend on the sample count, so unlike FID it can be read across sample sizes. Prompt alignment is the cosine
similarity between image and caption under OpenCLIP ViT-bigG-14, weights
\mbox{laion2b\_s39b\_b160k}~\cite{cherti2023reproducible,radford2021learning}. Precision, recall, density and coverage are computed from the same
Inception features with $k_\mathrm{nn} = 5$.
The memorisation audit uses the SSCD \mbox{disc-mixup} copy-detection
descriptor~\cite{pizzi2022self}. Per-prompt diversity uses LPIPS with its VGG
backbone~\cite{zhang2018unreasonable}, DreamSim~\cite{fu2023dreamsim} and the Vendi
score~\cite{friedman2023vendi} over DINOv2 features, on four samples for each of $1{,}000$ prompts.

\paragraph{What is held fixed between the two arms.}
Every comparison pairs \method against the same frozen backbone sampled from Gaussian noise, with
the same prompts and the same draw of $\veps$ per prompt from a fixed seed. Against the released
samplers the baseline keeps its own $50$ steps and guidance scale, $w = 1$ on Scale-RAE and $w = 4$ on
the other two. Unless a table states otherwise,
a cell uses $k = 50$, $\tau = 0.02$, $t_0 = 0.05$,
$N = 8$ and $w = 4$ over all $5{,}000$ held-out prompts of its dataset.
The per-prompt diversity cells use four samples for each of the
first $1{,}000$ of them.

\paragraph{Hardware.}
Every run used one NVIDIA RTX A5000 with $24$\,GiB. Retrieval
evaluates no generator, so the wall clock of a cell is set by the backbone's forward passes.


==> sections/app/C_qualitative.tex <==
\section{Qualitative results}
\label{app:qual}

\Cref{fig:supp_qual_coco,fig:supp_qual_anime,fig:supp_qual_art} compare the released sampler, RMG and \method on
every backbone and dataset of \cref{tab:main}, two prompts each.
\input{figures/sefi1024_qual/fig_sefi1024_qual}%
\input{figures/supp_qual/fig_supp_qual_coco}%
\input{figures/supp_qual/fig_supp_qual_art_anime}%


==> sections/app/D_ablations.tex <==
\section{Ablations}
\label{app:ablations}

\input{tables/ablation_seed/ablation_seed}

\paragraph{How many neighbours the anchor sees.}
Both $k$ and $\tau$ decide how many of the retrieved images make up the anchor and we sweep both in
\cref{tab:ablation}. At one extreme, $k = 1$ or $\tau \to 0$, the anchor is just the nearest
image. This gives the lowest FID on all three backbones but also the lowest diversity, which we
attribute to every sample of a prompt starting around the same real image (\cref{sec:exp:diversity}).
At the other extreme, $\tau = 0.1$, the weight spreads almost evenly over all $50$ neighbours
(\cref{fig:keff_hist}), so the anchor is close to their plain mean. Diversity is then the highest, but
FID goes up. Raising $k$ does not change much, because once $\tau$ is set (to $0.02$ in our case),
the anchor's weight on the far neighbours is negligible. In particular,
from $k = 25$ to $k = 200$ FID moves by at most $0.16$ on all three
backbones. We therefore fix $k = 50$ and use $\tau$ to move between the two extremes. We set
$\tau = 0.02$ as on Scale-RAE it gives the lowest FID while maintaining or increasing diversity against the
released sampler. LPIPS and
Vendi follow the DreamSim trend shown in the main paper (\cref{fig:div_keff_supp,fig:div_keff}).
SVG-T2I shows the same trend as Scale-RAE, while on
SeFi-Image FID and diversity barely change with $\tau$ (\cref{fig:keff_backbones}), possibly because the
anchor enters only its semantic latent.
\input{figures/keff_hist/fig_keff_hist}
\input{figures/div_keff_supp/fig_div_keff_supp}
\input{figures/keff_backbones/fig_keff_backbones}
\input{tables/u0/u0}
\input{tables/t0_knob/tab_t0_knob}%
\input{figures/pareto/fig_pareto}%
\edef\suppDpage{\the\value{page}}\newpage\loop\ifnum\value{page}<\numexpr\suppDpage+1\relax\null\newpage\repeat

\paragraph{The displacement $t_0$ and the guidance scale $w$.}
\Cref{tab:u0} sweeps both at $N = 8$ on Scale-RAE and SVG-T2I, with Gaussian sampling at the released
$50$ steps as the baseline. The two backbones do not agree on where the best $t_0$ is. Scale-RAE is best at
our default $t_0 = 0.05$ at every $w$ and loses ground quickly past it. SVG-T2I keeps improving past it
and is flat between $0.1$ and $0.2$, but that gain is bought with near-duplicates (\cref{tab:t0_knob}).
From $t_0 = 0.1$ the near-duplicate rate rises above the released sampler's on both backbones, and on
SVG-T2I it reaches $9.84\%$ at $t_0 = 0.2$, above the $3.82\%$ of real photographs.
On both, alignment falls steadily as $t_0$ grows and diversity peaks at
$t_0 = 0.05$. A smaller $t_0$ keeps more of the released sampler's alignment: on
SVG-T2I, $t_0 = 0.02$ reaches CLIP $0.439$ against $0.440$ and still lowers FID, $21.08$ against
$22.30$, but is less diverse than $t_0 = 0.05$. The sweep keeps the step count fixed, so every
scale above $w = 1$ takes two network evaluations per step. We use $w = 4$, the
released default of SVG-T2I and SeFi-Image, where \method on Scale-RAE also has its lowest FID. Comparing
the anchor and Gaussian noise at their own FID optima is misleading, because they reach those optima at
different alignments, so \cref{fig:pareto} plots FID against CLIP over the whole sweep. On SVG-T2I the
seeded curve lies below the Gaussian one across the whole shared range. On Scale-RAE the two ranges
barely meet, because at the same $w$ the anchor costs alignment. On Scale-RAE a reader who wants
maximum prompt adherence at any FID and step count should use guidance from noise, not a retrieval anchor.

\paragraph{A smaller store.}
\input{tables/pool/tab_pool}
The store is the one cost specific to \method. \Cref{tab:pool} measures what
a coarser one gives up, by pooling the retrieved latents over $P \times P$ token blocks before
\cref{eq:anchor}, which is numerically the same as storing a token grid $P$ times coarser. On
Scale-RAE FID grows and alignment falls steadily with $P$, and a store $16\times$ smaller still
reaches a lower FID than the released sampler, $27.84$ against $29.51$.
SVG-T2I is less sensitive to the pooling, up to $P = 4$ it matches the full store,
and a store $256\times$ smaller ($P = 16$) still scores $17.84$ against the released sampler's $22.30$.
On SeFi-Image the store almost has no effect on FID and stays within $0.16$ of the full store at every $P$,
though the store in SeFi-Image is already quite small compared to the other two ($6$--$18\times$ smaller).

\paragraph{Corpus density.}
\label{app:density}
\input{figures/density/fig_density}
The anchor is built from the prompt's retrieved neighbours, so the gain might depend on how
densely the corpus covers the prompt. We take the cosine similarity between a prompt and its
nearest corpus key as its density, split the $5{,}000$ prompts into five bins of about $1{,}000$,
and measure FID-1k in each bin (\cref{fig:density}).
A bin's FID-1k is over the $1{,}000$ corresponding images from the held-out set,
so it is larger than FID-5k and only comparable within the figure.
FID-1k rises as prompts get sparser for both samplers: from the densest bin to the sparsest by
$9.4$ (released sampler) and $10.6$ (\method) on Scale-RAE, and by $6.1$ and $8.7$ on SVG-T2I.
\method is lower than the released sampler in every bin, by $5.1$ to $7.7$ on Scale-RAE and $5.2$ to $7.8$ on SVG-T2I.
CLIP changes by less than $0.006$ per bin on
Scale-RAE. On SVG-T2I \method lowers it by $0.019$ in the sparsest bin and $0.002$ in the densest.


==> sections/app/E_anchor.tex <==
\section{Anchor ablations}
\label{app:anchor}

\subsection{Alternative anchors}
\label{app:anchor_controls}
\paragraph{Other anchors.}
\Cref{tab:anchor_app} gathers the controls of \cref{sec:exp:anchor}. The mean of the whole corpus, the
most ``corpus-typical'' point one might consider, is far worse than Gaussian sampling on both. The anchor
of a random prompt raises FID on both backbones and loses much of the alignment. A single corpus
latent drawn at random is worse as well, as it does not lower FID, $31.75$ against $29.51$ on Scale-RAE
and $23.01$ against $22.30$ on SVG-T2I, and it gives up most of the alignment, CLIP $0.244$ and
$0.270$ against $0.418$ and $0.440$. So the gain comes from the neighbours retrieved \textbf{for the prompt},
not from starting near the corpus. \Cref{fig:attribution} shows such an anchor, decoded, with the
retrieved images that contribute most to it.

\input{tables/anchor_control_app/tab_anchor_app}
\input{figures/attribution/fig_attribution}

\paragraph{Other noise.}
\label{app:isotropy}
\method keeps the noise $\veps$ of \cref{eq:state} isotropic. The alternative is to treat the $k$
retrieved latents as samples of a local distribution and draw the noise from the Gaussian they define,
\begin{equation}
  \begin{gathered}
    \tilde{\veps} = \sqrt{D}\, \frac{\bm{\xi}}{\lVert \bm{\xi} \rVert}, \qquad
    \bm{\xi} \sim \N(\vzero, \mSigma), \\
    \mSigma = \frac{1}{k - 1} \sum_{j \in \gI_k(\vq)} (\vz_j - \bar{\vz})(\vz_j - \bar{\vz})^\top
  \end{gathered}
  \label{eq:nbrnoise}
\end{equation}
where $\bar{\vz}$ is the plain mean of the $\vz_j$ and $D$ the dimension of the latent. $\mSigma$ is
their sample covariance, so $\bm{\xi}$ moves only along the $k - 1$ directions in which the neighbours
differ from each other. It is rescaled to $\sqrt{D}$, which is the norm a standard Gaussian
$\veps$ has in $D$ dimensions, so that only the directions of the noise change. $\tilde{\veps}$ then
replaces $\veps$ in \cref{eq:state}, and the anchor stays $\vmu$. This would theoretically help if the spread of
the neighbours said something about the prompt.
We test if the spectrum of the retrieved set is close to that of $k$ corpus latents
drawn at random using the participation ratio of the eigenvalues $\lambda_i$ of $\mSigma$, $\mathrm{PR} = (\sum_i \lambda_i)^2 / \sum_i \lambda_i^2$. Its value is
$k - 1$ for a flat spectrum and $1$ for a single direction.
The retrieved set's PR is $0.979$ of the random set's on Scale-RAE and $0.912$ on SVG-T2I at $k = 50$,
so the neighbours spread much like random latents and their spread says little about the prompt.
Accordingly, noise drawn in the span of the
neighbours costs $5.0$ FID and $0.059$ CLIP on Scale-RAE
and $12.9$ FID and $0.100$ CLIP on SVG-T2I (\cref{tab:nbrnoise}).

\input{tables/nbrnoise/tab_nbrnoise}

\subsection{Learned anchor}
\label{app:learned_anchor}
The learned anchor of \cref{tab:learned_anchor} is a proof of concept. It asks whether a network can
stand in for the store of the corpus. We did not optimize over its architecture or training recipe,
so this is what a first, untuned predictor reaches rather than the best a learned anchor can do. It
is a transformer encoder that maps the prompt's SigLIP-2 embedding $\vq$ to a latent of the
backbone's shape. A two-layer MLP with a GELU projects $\vq$ to width $512$. The result enters as a
prefix token and is also added to a learned position embedding for each output token, $256$ tokens
for Scale-RAE and SVG-T2I and $1{,}024$ for SeFi-Image. Six pre-norm layers of width $512$ follow,
with eight heads, a feed-forward width of $2{,}048$, GELU and no dropout, then a layer norm and a
linear head to the backbone's channels, $1{,}152$, $384$ and $16$. This gives $20.5$M, $20.1$M and
$20.3$M parameters, about $80$\,MiB each.

Training pairs every COCO train2017 caption with its image's latent from the store, over all
$118{,}287$ images, the same data \method retrieves from, with $2\%$ of the images held
out to monitor the fit. The loss is the mean squared error on latents standardised per channel, so
the network learns the expected latent given the caption. We use AdamW (learning rate
$3 \times 10^{-4}$, $\beta = (0.9, 0.99)$, weight decay $0.01$) with $500$ warm-up steps and cosine
decay, gradient clipping at $1$ and bfloat16 autocast, for $15{,}000$ steps at batch $256$. SeFi-Image,
with four times as many tokens, uses batch $128$ for $30{,}000$ steps.
At sampling time the prediction for the prompt, mapped back to the store's units, replaces $\vmu$,
with $t_0$, $N$, $w$ and $\veps$ unchanged.
It comes close to retrieval at the same $t_0$ and $N$, within $2.1$ FID on Scale-RAE and $0.2$ on
SVG-T2I and SeFi-Image, with a lower KID on the latter two (\cref{tab:learned_anchor}), which suggests
that what matters is the anchor more than how it was found. Unlike the store, however, it must be
retrained for every new corpus. \citet{ahn2024noise} take the learned route for the initial noise itself.
\input{tables/learned_anchor/tab_learned_anchor}


==> sections/app/F_limitations.tex <==
\section{Limitations}
\label{app:limitations}
\begin{itemize}[leftmargin=*, itemsep=2pt, topsep=2pt]
  \item \textbf{We depend on the impurity of the semantic space.} The mean of the retrieved latents
    stands for the prompt only when their impurity is low. Where it is high,
    as for SeFi-Image on Anime, \method might fall behind the released sampler in FID.
  \item \textbf{We need a captioned corpus.} Retrieval compares the prompt with the captions of the
    corpus, so an image collection without captions has to be captioned first.
  \item \textbf{Prompt length.} Retrieval embeds the prompt with SigLIP-2's text encoder, which reads
    $64$ tokens. Our prompts fit that limit, and a longer prompt would be
    truncated before retrieval.
  \item \textbf{Backbones.} On SeFi-Image \method seeds only the semantic latent and its
    texture latent starts from Gaussian noise, and there FID and diversity barely respond to $\tau$
    (\cref{fig:keff_backbones}).
\end{itemize}


==> tables/ablation_seed/ablation_seed.tex <==
\begin{table}[t]
  \centering
  \caption{\textbf{$\tau$ trades FID against diversity, and $k$ barely matters.} The nearest image alone ($k = 1$ or $\tau \to 0$) gives the lowest FID and the lowest diversity while $\tau = 0.1$ gives the highest diversity. From $k = 25$ to $k = 200$ FID changes little. All rows share $N = 8$, $w = 4$ and $t_0 = 0.05$, and differ only in how the $k$ retrieved latents are summarised. CLIP spans at most $0.010$ within a backbone. Shaded row is the default. Best per block in bold.}
  \label{tab:ablation}
  \setlength{\tabcolsep}{2pt}
  \small
  \begin{tabular}{lccccc}
    \toprule
    & FID $\downarrow$ & CLIP $\uparrow$ & LPIPS $\uparrow$ & DreamSim $\uparrow$ & Vendi $\uparrow$ \\
    \midrule
    \multicolumn{6}{l}{\textbf{Scale-RAE}} \\
    \multicolumn{6}{l}{\textit{$k$ nearest neighbours}} \\
    $k=1$ & \textbf{19.60} & 0.416 & 0.570 & 0.305 & 2.321 \\
    $k=5$ & 20.61 & 0.420 & 0.646 & 0.385 & 2.647 \\
    $k=25$ & 21.07 & \textbf{0.421} & 0.656 & 0.398 & 2.690 \\
    \rowcolor{gray!10}$k=50$ & 21.06 & 0.420 & 0.657 & 0.401 & 2.704 \\
    $k=200$ & 21.08 & 0.420 & \textbf{0.660} & \textbf{0.405} & \textbf{2.726} \\
    \cmidrule(l){2-6}
    \multicolumn{6}{l}{\textit{Temperature $\tau$}} \\
    $\tau \!\to\! 0$ & \textbf{19.52} & 0.416 & 0.570 & 0.305 & 2.320 \\
    $\tau = 0.003$ & 19.74 & 0.418 & 0.595 & 0.330 & 2.432 \\
    $\tau = 0.01$ & 20.17 & \textbf{0.420} & 0.635 & 0.375 & 2.595 \\
    \rowcolor{gray!10}$\tau = 0.02$ & 21.06 & \textbf{0.420} & 0.657 & 0.401 & 2.704 \\
    $\tau = 0.03$ & 22.82 & 0.417 & 0.665 & 0.411 & 2.749 \\
    $\tau = 0.1$ & 23.30 & 0.414 & \textbf{0.669} & \textbf{0.420} & \textbf{2.782} \\
    \midrule
    \multicolumn{6}{l}{\textbf{SVG-T2I}} \\
    \multicolumn{6}{l}{\textit{$k$ nearest neighbours}} \\
    $k=1$ & \textbf{16.82} & 0.423 & 0.589 & 0.311 & 2.336 \\
    $k=5$ & 16.84 & \textbf{0.430} & 0.647 & 0.359 & 2.516 \\
    $k=25$ & 16.98 & \textbf{0.430} & 0.656 & 0.367 & 2.557 \\
    \rowcolor{gray!10}$k=50$ & 16.96 & \textbf{0.430} & 0.657 & 0.370 & 2.567 \\
    $k=200$ & 16.99 & \textbf{0.430} & \textbf{0.660} & \textbf{0.372} & \textbf{2.581} \\
    \cmidrule(l){2-6}
    \multicolumn{6}{l}{\textit{Temperature $\tau$}} \\
    $\tau \!\to\! 0$ & \textbf{16.84} & 0.423 & 0.589 & 0.311 & 2.333 \\
    $\tau = 0.003$ & 16.88 & 0.425 & 0.608 & 0.326 & 2.384 \\
    $\tau = 0.01$ & 16.92 & 0.427 & 0.639 & 0.351 & 2.494 \\
    \rowcolor{gray!10}$\tau = 0.02$ & 16.96 & 0.430 & 0.657 & 0.370 & 2.567 \\
    $\tau = 0.03$ & 17.41 & \textbf{0.433} & 0.664 & 0.376 & 2.594 \\
    $\tau = 0.1$ & 17.63 & 0.431 & \textbf{0.669} & \textbf{0.383} & \textbf{2.626} \\
    \midrule
    \multicolumn{6}{l}{\textbf{SeFi-Image}} \\
    \multicolumn{6}{l}{\textit{$k$ nearest neighbours}} \\
    $k=1$ & \textbf{31.31} & \textbf{0.397} & 0.654 & 0.373 & 2.578 \\
    $k=5$ & 31.64 & 0.395 & 0.660 & 0.379 & 2.592 \\
    $k=25$ & 31.57 & 0.396 & 0.661 & 0.381 & 2.603 \\
    \rowcolor{gray!10}$k=50$ & 31.60 & 0.395 & 0.662 & 0.382 & 2.606 \\
    $k=200$ & 31.73 & 0.395 & \textbf{0.663} & \textbf{0.384} & \textbf{2.613} \\
    \cmidrule(l){2-6}
    \multicolumn{6}{l}{\textit{Temperature $\tau$}} \\
    $\tau \!\to\! 0$ & \textbf{31.32} & \textbf{0.397} & 0.656 & 0.375 & 2.582 \\
    $\tau = 0.003$ & 31.47 & 0.396 & 0.658 & 0.376 & 2.585 \\
    \rowcolor{gray!10}$\tau = 0.02$ & 31.60 & 0.395 & 0.662 & 0.382 & 2.606 \\
    $\tau = 0.03$ & 31.58 & 0.395 & 0.663 & 0.383 & 2.612 \\
    $\tau = 0.1$ & 31.72 & 0.394 & \textbf{0.664} & \textbf{0.386} & \textbf{2.620} \\
    \bottomrule
  \end{tabular}
\end{table}


==> tables/anchor_control_app/tab_anchor_app.tex <==
\begin{table}[!h]
  \centering
  \caption{\textbf{Anchors that are not the prompt's own.} Only the prompt's own anchor (\method) beats the released sampler in FID, and every other anchor is worse than it in both FID and CLIP. Each anchor replaces $\vmu$ in \cref{eq:state} with nothing else changed.
  \emph{Global corpus mean} is the mean latent of the whole corpus.
  \emph{Random prompt} is the anchor retrieved for another randomly drawn prompt.
  \emph{Random image} is the latent of one corpus image drawn at random.
  Best per column in bold.
  }
  \label{tab:anchor_app}
  \setlength{\tabcolsep}{2pt}
  \begin{tabular}{lcccc}
    \toprule
    & \multicolumn{2}{c}{Scale-RAE} & \multicolumn{2}{c}{SVG-T2I} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
    What is the \emph{Anchor}? & FID $\downarrow$ & CLIP $\uparrow$ & FID $\downarrow$ & CLIP $\uparrow$ \\
    \midrule
    No anchor (Baseline) & 29.51 & 0.418 & 22.30 & \textbf{0.440} \\
    Global corpus mean & 49.45 & 0.323 & 38.18 & 0.380 \\
    Random prompt & 38.63 & 0.274 & 24.66 & 0.293 \\
    Random image & 31.75 & 0.244 & 23.01 & 0.270 \\
    \midrule
    \rowcolor{gray!10}Regular (\method) & \textbf{21.06} & \textbf{0.420} & \textbf{16.96} & 0.430 \\
    \bottomrule
  \end{tabular}
\end{table}


==> tables/app_prdc/app_prdc.tex <==
\begin{table*}[t]
  \centering
  \caption{\textbf{\method is comparable to or better than Gaussian sampling all around.} At every step budget it has a
  lower FID and a higher recall and coverage, its precision and density are higher or within $0.025$, and its CLIP is
  within $0.012$. Gaussian sampling, RMG and \method at each budget on COCO held-out prompts. Precision, recall, density and coverage are from the same features with $k_\mathrm{nn} = 5$.
  Precision and density measure fidelity to the reference manifold, recall and coverage measure how much of it is reached.
  At each budget the best of the three sources is in bold.}
  \label{tab:app_prdc}
  \setlength{\tabcolsep}{2pt}
  \footnotesize
  \setlength{\aboverulesep}{0pt}\setlength{\belowrulesep}{0pt}\setlength{\extrarowheight}{1.5pt}
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{cl|cccccc|cccccc|cccccc}
    \toprule
    & & \multicolumn{6}{c|}{Scale-RAE} & \multicolumn{6}{c|}{SVG-T2I} & \multicolumn{6}{c}{SeFi-Image} \\
    \cmidrule(lr){3-8} \cmidrule(lr){9-14} \cmidrule(lr){15-20}
    Steps & Source & FID $\downarrow$ & CLIP $\uparrow$ & Prec. $\uparrow$ & Rec. $\uparrow$ & Dens. $\uparrow$ & Cov. $\uparrow$ & FID $\downarrow$ & CLIP $\uparrow$ & Prec. $\uparrow$ & Rec. $\uparrow$ & Dens. $\uparrow$ & Cov. $\uparrow$ & FID $\downarrow$ & CLIP $\uparrow$ & Prec. $\uparrow$ & Rec. $\uparrow$ & Dens. $\uparrow$ & Cov. $\uparrow$ \\
    \midrule
    & Gaussian & 33.03 & 0.418 & 0.681 & 0.496 & 0.672 & 0.764 & 26.81 & \textbf{0.436} & 0.735 & 0.571 & 0.926 & 0.855 & 47.36 & 0.373 & 0.498 & 0.463 & 0.400 & 0.567 \\
    & + RMG & 34.62 & \textbf{0.434} & 0.671 & 0.475 & 0.630 & 0.734 & 25.27 & 0.421 & 0.758 & 0.548 & 0.974 & 0.895 & 58.13 & 0.347 & 0.433 & 0.460 & 0.329 & 0.506 \\
    \rowcolor{gray!10}\multirow{-3}{*}{4} & + \method & \textbf{22.27} & 0.418 & \textbf{0.694} & \textbf{0.651} & \textbf{0.750} & \textbf{0.873} & \textbf{18.14} & 0.431 & \textbf{0.812} & \textbf{0.624} & \textbf{1.161} & \textbf{0.950} & \textbf{41.60} & \textbf{0.376} & \textbf{0.561} & \textbf{0.465} & \textbf{0.510} & \textbf{0.654} \\
    \midrule
    & Gaussian & 30.27 & 0.421 & 0.730 & 0.503 & 0.796 & 0.819 & 23.73 & \textbf{0.441} & 0.754 & 0.607 & 0.955 & 0.881 & 35.32 & \textbf{0.404} & \textbf{0.716} & 0.475 & 0.813 & 0.776 \\
    & + RMG & 30.49 & \textbf{0.437} & \textbf{0.735} & 0.486 & 0.766 & 0.802 & 19.90 & 0.430 & 0.807 & 0.606 & \textbf{1.205} & 0.946 & 34.85 & 0.380 & 0.655 & 0.488 & 0.755 & 0.774 \\
    \rowcolor{gray!10}\multirow{-3}{*}{8} & + \method & \textbf{21.06} & 0.420 & 0.714 & \textbf{0.651} & \textbf{0.814} & \textbf{0.888} & \textbf{16.96} & 0.430 & \textbf{0.822} & \textbf{0.631} & 1.202 & \textbf{0.956} & \textbf{31.60} & 0.395 & 0.711 & \textbf{0.493} & \textbf{0.834} & \textbf{0.805} \\
    \midrule
    & Gaussian & 29.50 & 0.420 & 0.744 & 0.504 & 0.828 & 0.834 & 22.87 & \textbf{0.441} & 0.754 & 0.632 & 0.935 & 0.874 & 36.47 & \textbf{0.407} & \textbf{0.757} & 0.430 & \textbf{0.939} & 0.798 \\
    & + RMG & 29.27 & \textbf{0.437} & \textbf{0.746} & 0.496 & 0.801 & 0.824 & 18.94 & 0.429 & \textbf{0.825} & 0.597 & \textbf{1.259} & 0.958 & \textbf{31.82} & 0.388 & 0.718 & \textbf{0.482} & 0.881 & \textbf{0.808} \\
    \rowcolor{gray!10}\multirow{-3}{*}{16} & + \method & \textbf{20.72} & 0.420 & 0.719 & \textbf{0.648} & \textbf{0.833} & \textbf{0.896} & \textbf{16.46} & 0.429 & 0.812 & \textbf{0.642} & 1.202 & \textbf{0.959} & 32.20 & 0.396 & 0.746 & 0.467 & 0.923 & 0.805 \\
    \midrule
    & Gaussian & 29.51 & 0.418 & 0.728 & 0.520 & \textbf{0.797} & 0.816 & 22.30 & \textbf{0.440} & 0.754 & 0.637 & 0.955 & 0.887 & 37.32 & \textbf{0.406} & \textbf{0.768} & 0.414 & \textbf{1.006} & 0.804 \\
    & + RMG & 30.41 & \textbf{0.434} & \textbf{0.731} & 0.494 & 0.761 & 0.810 & 18.30 & 0.428 & \textbf{0.825} & 0.624 & \textbf{1.235} & 0.958 & \textbf{31.51} & 0.389 & 0.744 & \textbf{0.458} & 0.950 & \textbf{0.823} \\
    \rowcolor{gray!10}\multirow{-3}{*}{50} & + \method & \textbf{21.77} & 0.418 & 0.714 & \textbf{0.642} & 0.796 & \textbf{0.879} & \textbf{16.17} & 0.428 & 0.812 & \textbf{0.647} & 1.208 & \textbf{0.963} & 32.86 & 0.396 & 0.763 & 0.434 & 1.003 & 0.816 \\
    \bottomrule
  \end{tabular}}
\end{table*}


==> tables/fd_cmmd/fd_cmmd.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.1}
\caption{\textbf{\method's gain holds in DINOv2 and CLIP feature spaces.} It has the lowest FD$_\text{DINOv2}$ in all nine settings and the lowest CMMD in eight. FD$_\text{DINOv2}$ and CMMD for the runs of \cref{tab:main}, against the same held-out reference images, lower is better.}
\label{tab:fd_cmmd}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{2}{c}{COCO} & \multicolumn{2}{c}{Anime} & \multicolumn{2}{c}{WikiArt} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
Method & FD$_\text{DINOv2}$$\downarrow$ & CMMD$\downarrow$ & FD$_\text{DINOv2}$$\downarrow$ & CMMD$\downarrow$ & FD$_\text{DINOv2}$$\downarrow$ & CMMD$\downarrow$ \\
\midrule
\multicolumn{7}{l}{\textit{Scale-RAE}} \\
Baseline & 470.7 & 0.570 & 255.3 & 1.034 & 661.4 & 1.348 \\
+ RMG~\cite{curvo2026follow} & 462.4 & 0.729 & 626.0 & 2.289 & 371.7 & 1.029 \\
\cellcolor{gray!10}+ \method{} (ours) & \cellcolor{gray!10}\textbf{373.1} & \cellcolor{gray!10}\textbf{0.454} & \cellcolor{gray!10}\textbf{208.6} & \cellcolor{gray!10}\textbf{0.715} & \cellcolor{gray!10}\textbf{225.6} & \cellcolor{gray!10}\textbf{0.530} \\
\midrule
\multicolumn{7}{l}{\textit{SVG-T2I}} \\
Baseline & 358.9 & 0.489 & 825.3 & 1.860 & 468.0 & 1.013 \\
+ RMG~\cite{curvo2026follow} & 379.6 & 0.674 & 694.1 & 1.740 & 331.9 & 0.852 \\
\cellcolor{gray!10}+ \method{} (ours) & \cellcolor{gray!10}\textbf{311.9} & \cellcolor{gray!10}\textbf{0.471} & \cellcolor{gray!10}\textbf{559.7} & \cellcolor{gray!10}\textbf{1.628} & \cellcolor{gray!10}\textbf{261.0} & \cellcolor{gray!10}\textbf{0.844} \\
\midrule
\multicolumn{7}{l}{\textit{SeFi-Image}} \\
Baseline & 475.1 & \textbf{0.559} & 553.7 & 1.449 & 883.7 & 1.457 \\
+ RMG~\cite{curvo2026follow} & 491.6 & 0.579 & 549.1 & 1.469 & 801.2 & 1.379 \\
\cellcolor{gray!10}+ \method{} (ours) & \cellcolor{gray!10}\textbf{470.6} & \cellcolor{gray!10}0.602 & \cellcolor{gray!10}\textbf{540.4} & \cellcolor{gray!10}\textbf{1.337} & \cellcolor{gray!10}\textbf{726.0} & \cellcolor{gray!10}\textbf{1.282} \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/latency/tab_latency.tex <==
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{1.8pt}
\renewcommand{\arraystretch}{1.1}
\caption{\textbf{Latency.} How much faster is \method in wall-clock time? Median wall clock per prompt on one RTX A5000, the released sampler at $50$ steps, RMG at $20$ and \method at $8$, with speedups relative to the measured time of the released sampler. The one-time read takes at most $7$\,ms.}
\label{tab:latency}
\begin{tabular}{lcccccc}
\toprule
 & \multirow{3}{*}{\makecell{One-Time\\Read (s)}} & \multicolumn{5}{c}{Sampling (s)} \\
\cmidrule(lr){3-7}
 & & \multirow{2}{*}{Released} & \multicolumn{2}{c}{RMG} & \multicolumn{2}{c}{\method} \\
\cmidrule(lr){4-5} \cmidrule(lr){6-7}
Backbone & & & Time & Speedup & Time & Speedup \\
\midrule
Scale-RAE (serial) & 0.004 & 1.60 & 1.31 & 1.23$\times$ & 0.51 & 3.15$\times$ \\
SVG-T2I & 0.007 & 3.12 & 1.25 & 2.50$\times$ & 0.50 & 6.24$\times$ \\
SeFi-Image & 0.002 & 13.83 & 5.52 & 2.51$\times$ & 2.22 & 6.23$\times$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/learned_anchor/tab_learned_anchor.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.1}
\caption{\textbf{A learned anchor in place of retrieval.} It comes within $2.1$ FID of \method, but must be retrained for every new corpus. A network trained on the COCO train2017 caption and latent pairs predicts $\vmu$ from the prompt, with FID-5k, KID and CLIP over the 5{,}000 COCO val2017 captions as in \cref{tab:main}.}
\label{tab:learned_anchor}
\begin{tabular}{lccccc}
\toprule
Method & Steps & \makecell{Training-\\free?} & FID$\downarrow$ & KID{\scriptsize$\times 10^3$}$\downarrow$ & CLIP$\uparrow$ \\
\midrule
\multicolumn{6}{l}{\textit{Scale-RAE}} \\
Baseline & 50 & \na & 29.51 & 7.77 & 0.418 \\
+ Learned anchor & 8 & \xmark & 23.11 & 3.66 & 0.418 \\
\cellcolor{gray!10}+ \method{} (ours) & \cellcolor{gray!10}8 & \cellcolor{gray!10}\cmark & \cellcolor{gray!10}\textbf{21.06} & \cellcolor{gray!10}\textbf{3.20} & \cellcolor{gray!10}\textbf{0.420} \\
\midrule
\multicolumn{6}{l}{\textit{SVG-T2I}} \\
Baseline & 50 & \na & 22.30 & 3.83 & \textbf{0.440} \\
+ Learned anchor & 8 & \xmark & 17.12 & \textbf{1.56} & 0.435 \\
\cellcolor{gray!10}+ \method{} (ours) & \cellcolor{gray!10}8 & \cellcolor{gray!10}\cmark & \cellcolor{gray!10}\textbf{16.96} & \cellcolor{gray!10}1.73 & \cellcolor{gray!10}0.430 \\
\midrule
\multicolumn{6}{l}{\textit{SeFi-Image}} \\
Baseline & 50 & \na & 37.32 & 12.02 & \textbf{0.406} \\
+ Learned anchor & 8 & \xmark & 31.74 & \textbf{7.56} & 0.395 \\
\cellcolor{gray!10}+ \method{} (ours) & \cellcolor{gray!10}8 & \cellcolor{gray!10}\cmark & \cellcolor{gray!10}\textbf{31.60} & \cellcolor{gray!10}7.70 & \cellcolor{gray!10}0.395 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/memorization/memorization.tex <==
\begin{table}[t]
  \centering
  \caption{\textbf{\method does not copy its retrieved images.}
  At most $0.32\%$ of its images cross the copy threshold, close to the released sampler.
  Maximum SSCD similarity of each generation to its dataset's corpus (top-1)
  and the share above the copy threshold of $0.5$,
  for the runs of \cref{tab:main}.
  Held-out images are the real image of each prompt, scored the same way.
  The lowest of the three sources per backbone is in bold.}
  \label{tab:memorization}
  \setlength{\tabcolsep}{1.5pt}
  \footnotesize
  \begin{tabular}{lcccccc}
    \toprule
    & \multicolumn{2}{c}{COCO} & \multicolumn{2}{c}{Anime} & \multicolumn{2}{c}{WikiArt} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
    Source & top-1$\downarrow$ & \% $> 0.5{\downarrow}$ & top-1$\downarrow$ & \% $> 0.5{\downarrow}$ & top-1$\downarrow$ & \% $> 0.5{\downarrow}$ \\
    \midrule
    Held-out images & 0.286 & 3.82 & 0.393 & 6.00 & 0.329 & 4.04 \\
    \midrule
    \multicolumn{7}{@{}l}{\textit{Scale-RAE}} \\
    Baseline & 0.256 & \textbf{0.00} & \textbf{0.323} & \textbf{0.04} & \textbf{0.246} & \textbf{0.14} \\
    + RMG & 0.257 & \textbf{0.00} & 0.369 & 1.10 & 0.278 & 0.34 \\
    \rowcolor{gray!10}+ \method & \textbf{0.254} & \textbf{0.00} & 0.341 & \textbf{0.04} & 0.284 & 0.20 \\
    \midrule
    \multicolumn{7}{@{}l}{\textit{SVG-T2I}} \\
    Baseline & \textbf{0.259} & 0.04 & \textbf{0.285} & \textbf{0.00} & \textbf{0.253} & \textbf{0.10} \\
    + RMG & 0.262 & \textbf{0.02} & 0.299 & 0.06 & 0.268 & 0.28 \\
    \rowcolor{gray!10}+ \method & 0.260 & \textbf{0.02} & 0.318 & 0.16 & 0.269 & \textbf{0.10} \\
    \midrule
    \multicolumn{7}{@{}l}{\textit{SeFi-Image}} \\
    Baseline & 0.264 & 0.10 & 0.335 & 0.44 & 0.247 & \textbf{0.24} \\
    + RMG & 0.255 & 0.04 & 0.325 & \textbf{0.16} & \textbf{0.246} & 0.30 \\
    \rowcolor{gray!10}+ \method & \textbf{0.254} & \textbf{0.02} & \textbf{0.321} & 0.24 & 0.256 & 0.32 \\
    \bottomrule
  \end{tabular}
\end{table}


==> tables/nbrnoise/tab_nbrnoise.tex <==
\begin{table}[!h]
  \centering
  \caption{\textbf{Noise shaped by the neighbourhood.} It is worse than isotropic noise in both FID and CLIP. The isotropic $\veps$ of \cref{eq:state} replaced by a draw in the span of the $k$ retrieved latents at the same norm. Best per column in bold.}
  \label{tab:nbrnoise}
  \setlength{\tabcolsep}{2pt}
  \small
  \begin{tabular}{lcccc}
    \toprule
    & \multicolumn{2}{c}{Scale-RAE} & \multicolumn{2}{c}{SVG-T2I} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
    Noise & FID $\downarrow$ & CLIP $\uparrow$ & FID $\downarrow$ & CLIP $\uparrow$ \\
    \midrule
    Baseline & 29.51 & 0.418 & 22.30 & \textbf{0.440} \\
    + Neighbour $\veps$ & 26.05 & 0.361 & 29.84 & 0.330 \\
    \rowcolor{gray!10}+ \method (isotropic $\veps$) & \textbf{21.06} & \textbf{0.420} & \textbf{16.96} & 0.430 \\
    \bottomrule
  \end{tabular}
\end{table}


==> tables/pool/tab_pool.tex <==
\begin{table}[t]
  \centering
  \caption{\textbf{A coarser latent store.} A store $16\times$ smaller still beats the released sampler on all three backbones. The $k$ retrieved latents are average-pooled over $P \times P$ token blocks before \cref{eq:anchor}, as a store $P^2$ times smaller would return them. Store is the size for COCO train2017 latents. Best per column in bold.}
  \label{tab:pool}
  \setlength{\tabcolsep}{1.5pt}
  \footnotesize
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{lccccccccc}
    \toprule
    & \multicolumn{3}{c}{Scale-RAE} & \multicolumn{3}{c}{SVG-T2I} & \multicolumn{3}{c}{SeFi-Image} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
    & \makecell{Store\\(GiB)} & FID $\downarrow$ & CLIP $\uparrow$ & \makecell{Store\\(GiB)} & FID $\downarrow$ & CLIP $\uparrow$ & \makecell{Store\\(GiB)} & FID $\downarrow$ & CLIP $\uparrow$ \\
    \midrule
    Baseline & $-$ & 29.51 & 0.418 & $-$ & 22.30 & \textbf{0.440} & $-$ & 37.32 & \textbf{0.406} \\
    $P = 16$ & 0.25 & 36.13 & 0.390 & 0.085 & 17.84 & 0.426 & 0.014 & 31.76 & 0.383 \\
    $P = 8$ & 1.0 & 32.17 & 0.397 & 0.34 & 17.10 & 0.428 & 0.056 & \textbf{31.52} & 0.391 \\
    $P = 4$ & 4.1 & 27.84 & 0.406 & 1.4 & \textbf{16.86} & 0.430 & 0.23 & 31.60 & 0.394 \\
    $P = 2$ & 16.2 & 24.50 & 0.412 & 5.4 & 16.88 & 0.430 & 0.90 & \textbf{31.52} & 0.395 \\
    \rowcolor{gray!10}\method, $P = 1$ & 65.0 & \textbf{21.06} & \textbf{0.420} & 21.7 & 16.96 & 0.430 & 3.6 & 31.60 & 0.395 \\
    \bottomrule
  \end{tabular}}
\end{table}


==> tables/rmg_k20/tab_rmg_k20.tex <==
\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.1}
\caption{\textbf{\method's lead over RMG does not come from reading more images.} With both reading the same $k$ retrieved COCO train2017 images per prompt, \method has the lower FID and KID on Scale-RAE and SVG-T2I at $k = 20$ and $k = 50$, and the two are almost level on SeFi-Image. Over the $5{,}000$ COCO val2017 prompts, with each method at its default number of steps.}
\label{tab:app_rmg}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lc|cccccc|cccccc}
\toprule
 & & \multicolumn{6}{c|}{Bank / nearest neighbours $k = 20$} & \multicolumn{6}{c}{Bank / nearest neighbours $k = 50$} \\
\cmidrule(lr){3-8} \cmidrule(lr){9-14}
 & & \multicolumn{3}{c}{Fidelity and alignment} & \multicolumn{3}{c|}{Per-prompt diversity} & \multicolumn{3}{c}{Fidelity and alignment} & \multicolumn{3}{c}{Per-prompt diversity} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
Method & Speedup$\uparrow$ & FID$\downarrow$ & KID{\scriptsize$\times 10^3$}$\downarrow$ & CLIP$\uparrow$ & LPIPS$\uparrow$ & DreamSim$\uparrow$ & Vendi$\uparrow$ & FID$\downarrow$ & KID{\scriptsize$\times 10^3$}$\downarrow$ & CLIP$\uparrow$ & LPIPS$\uparrow$ & DreamSim$\uparrow$ & Vendi$\uparrow$ \\
\midrule
\multicolumn{2}{l|}{\textit{Scale-RAE}} & & & & & & & & & & & & \\
Baseline & $\times$1 & 29.51 & 7.77 & 0.418 & \textbf{0.664} & 0.385 & 2.634 & 29.51 & 7.77 & 0.418 & \textbf{0.664} & 0.385 & 2.634 \\
+ RMG~\cite{curvo2026follow} & $\times$2.5 & 29.36 & 6.93 & \textbf{0.436} & 0.593 & 0.286 & 2.294 & 29.70 & 6.96 & \textbf{0.436} & 0.595 & 0.287 & 2.302 \\
\rowcolor{gray!10}+ \method{} (ours) & \textbf{\boldmath$\times$6.25} & \textbf{20.95} & \textbf{3.17} & 0.421 & 0.654 & \textbf{0.396} & \textbf{2.679} & \textbf{21.06} & \textbf{3.20} & 0.420 & 0.657 & \textbf{0.401} & \textbf{2.704} \\
\midrule
\multicolumn{2}{l|}{\textit{SVG-T2I}} & & & & & & & & & & & & \\
Baseline & $\times$1 & 22.30 & 3.83 & \textbf{0.440} & 0.652 & 0.336 & 2.384 & 22.30 & 3.83 & \textbf{0.440} & 0.652 & 0.336 & 2.384 \\
+ RMG~\cite{curvo2026follow} & $\times$2.5 & 18.73 & 2.17 & 0.429 & 0.626 & 0.330 & 2.430 & 19.02 & 2.27 & 0.429 & 0.628 & 0.332 & 2.448 \\
\rowcolor{gray!10}+ \method{} (ours) & \textbf{\boldmath$\times$6.25} & \textbf{16.98} & \textbf{1.74} & 0.430 & \textbf{0.653} & \textbf{0.364} & \textbf{2.547} & \textbf{16.96} & \textbf{1.73} & 0.430 & \textbf{0.657} & \textbf{0.370} & \textbf{2.567} \\
\midrule
\multicolumn{2}{l|}{\textit{SeFi-Image}} & & & & & & & & & & & & \\
Baseline & $\times$1 & 37.32 & 12.02 & \textbf{0.406} & 0.650 & 0.323 & 2.259 & 37.32 & 12.02 & \textbf{0.406} & 0.650 & 0.323 & 2.259 \\
+ RMG~\cite{curvo2026follow} & $\times$2.5 & 31.70 & \textbf{7.42} & 0.388 & \textbf{0.663} & \textbf{0.387} & \textbf{2.654} & 31.93 & \textbf{7.44} & 0.387 & \textbf{0.664} & \textbf{0.388} & \textbf{2.656} \\
\rowcolor{gray!10}+ \method{} (ours) & \textbf{\boldmath$\times$6.25} & \textbf{31.62} & 7.73 & 0.395 & 0.661 & 0.381 & 2.598 & \textbf{31.60} & 7.70 & 0.395 & 0.662 & 0.382 & 2.606 \\
\bottomrule
\end{tabular}}
\end{table*}


==> tables/solver/tab_solver.tex <==
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.1}
\caption{\textbf{Euler and DPM-Solver++(2M) at $N = 8$.} FID, KID and CLIP on COCO for Gaussian sampling and \method, each integrated with either solver. The gain is nearly the same with both solvers.}
\label{tab:solver}
\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{3}{c}{Euler} & \multicolumn{3}{c}{DPM-Solver++} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
Method & FID$\downarrow$ & KID{\scriptsize$\times 10^3$}$\downarrow$ & CLIP$\uparrow$ & FID$\downarrow$ & KID{\scriptsize$\times 10^3$}$\downarrow$ & CLIP$\uparrow$ \\
\midrule
\multicolumn{7}{l}{\textit{Scale-RAE}} \\
Gaussian & 30.27 & 8.85 & \textbf{0.421} & 29.43 & 8.44 & \textbf{0.421} \\
\cellcolor{gray!10}\method & \cellcolor{gray!10}\textbf{21.06} & \cellcolor{gray!10}\textbf{3.20} & \cellcolor{gray!10}0.420 & \cellcolor{gray!10}\textbf{20.29} & \cellcolor{gray!10}\textbf{2.94} & \cellcolor{gray!10}0.420 \\
\midrule
\multicolumn{7}{l}{\textit{SVG-T2I}} \\
Gaussian & 23.73 & 4.71 & \textbf{0.441} & 23.09 & 4.31 & \textbf{0.440} \\
\cellcolor{gray!10}\method & \cellcolor{gray!10}\textbf{16.96} & \cellcolor{gray!10}\textbf{1.73} & \cellcolor{gray!10}0.430 & \cellcolor{gray!10}\textbf{16.54} & \cellcolor{gray!10}\textbf{1.46} & \cellcolor{gray!10}0.428 \\
\midrule
\multicolumn{7}{l}{\textit{SeFi-Image}} \\
Gaussian & 35.32 & 10.14 & \textbf{0.404} & 35.12 & 9.78 & \textbf{0.403} \\
\cellcolor{gray!10}\method & \cellcolor{gray!10}\textbf{31.60} & \cellcolor{gray!10}\textbf{7.70} & \cellcolor{gray!10}0.395 & \cellcolor{gray!10}\textbf{31.24} & \cellcolor{gray!10}\textbf{7.38} & \cellcolor{gray!10}0.395 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/store_size/tab_store_size.tex <==
\begin{table}[t]
  \centering
  \caption{\textbf{Store sizes.} The fp16 corpus latents kept in each backbone's latent space and the SigLIP-2 caption keys that all three share.}
  \label{tab:store_size}
  \setlength{\tabcolsep}{1.5pt}
  \footnotesize
  \begin{tabular}{lcrrrr}
    \toprule
    Store & Shape & Per image & COCO & Anime & WikiArt \\
    \midrule
    Images & & & 118{,}287 & 120{,}810 & 69{,}521 \\
    \midrule
    Scale-RAE & 256$\,\times\,$1152 & 576\,KiB & 64.98\,GiB & 66.36\,GiB & 38.19\,GiB \\
    SVG-T2I & 256$\,\times\,$384 & 192\,KiB & 21.66\,GiB & 22.12\,GiB & 12.73\,GiB \\
    SeFi-Image & 1024$\,\times\,$16 & 32\,KiB & 3.61\,GiB & 3.69\,GiB & 2.12\,GiB \\
    \midrule
    SigLIP-2 keys & 1152 & 2.25\,KiB & 0.25\,GiB & 0.26\,GiB & 0.15\,GiB \\
    \bottomrule
  \end{tabular}
\end{table}


==> tables/t0_knob/tab_t0_knob.tex <==
\begin{table}[t]
  \centering
  \caption{\textbf{Past $t_0 = 0.05$, \method copies more and aligns less.} From $t_0 = 0.1$ the near-duplicate rate rises above the released sampler's, CLIP falls steadily and diversity peaks at $t_0 = 0.05$. \method as $t_0$ grows, with per-prompt diversity and the near-duplicate rate~\cite{somepalli2023diffusion} (real photographs: $3.82\%$). $t_0 = 0$ is Gaussian noise like the released sampler (but at $w=4$). The shaded row is the default. Best per column within a block in bold.}
  \label{tab:t0_knob}
  \setlength{\tabcolsep}{1.5pt}
  \footnotesize
  \begin{tabular}{@{}clcccccc@{}}
    \toprule
    & $t_0$ & FID $\downarrow$ & CLIP $\uparrow$ & LPIPS $\uparrow$ & DreamSim $\uparrow$ & Vendi $\uparrow$ & Near-dup.\,\% $\downarrow$ \\
    \midrule
     & $0$ & 32.53 & \textbf{0.448} & 0.572 & 0.245 & 2.07 & \textbf{0.00} \\
     & $0.02$ & 27.95 & 0.442 & 0.630 & 0.320 & 2.34 & \textbf{0.00} \\
     & \cellcolor{gray!10}$0.05$ & \cellcolor{gray!10}\textbf{21.06} & \cellcolor{gray!10}0.420 & \cellcolor{gray!10}\textbf{0.657} & \cellcolor{gray!10}\textbf{0.401} & \cellcolor{gray!10}\textbf{2.70} & \cellcolor{gray!10}\textbf{0.00} \\
     & $0.1$ & 22.84 & 0.394 & 0.626 & 0.371 & 2.68 & 0.26 \\
    \multirow{-5}{*}{\rotatebox[origin=c]{90}{\textbf{Scale-RAE}}} & $0.2$ & 27.73 & 0.374 & 0.563 & 0.274 & 2.44 & 3.32 \\
    \midrule
     & $0$ & 22.30 & \textbf{0.440} & 0.652 & 0.336 & 2.38 & 0.04 \\
     & $0.02$ & 21.08 & 0.439 & 0.655 & 0.348 & 2.45 & \textbf{0.02} \\
     & \cellcolor{gray!10}$0.05$ & \cellcolor{gray!10}16.96 & \cellcolor{gray!10}0.430 & \cellcolor{gray!10}\textbf{0.657} & \cellcolor{gray!10}\textbf{0.370} & \cellcolor{gray!10}\textbf{2.57} & \cellcolor{gray!10}\textbf{0.02} \\
     & $0.1$ & 15.44 & 0.414 & 0.631 & 0.341 & 2.49 & 0.48 \\
    \multirow{-5}{*}{\rotatebox[origin=c]{90}{\textbf{SVG-T2I}}} & $0.2$ & \textbf{15.29} & 0.397 & 0.586 & 0.283 & 2.32 & 9.84 \\
    \bottomrule
  \end{tabular}
\end{table}


==> tables/u0/u0.tex <==
\begin{table*}[t]
  \centering
  \caption{\textbf{The best $t_0$ depends on the backbone and desired properties.} Scale-RAE has its lowest FID at our default $t_0 = 0.05$ at every $w$, while SVG-T2I keeps improving past it. FID-5k and CLIP at $N = 8$ as the displacement $t_0$ of \cref{eq:state} and the guidance scale $w$ vary. Baseline is Gaussian noise at the released 50 steps, at each $w$. The shaded row is the default. Best per column within a block in bold.}
  \label{tab:u0}\label{tab:guidance}
  \setlength{\tabcolsep}{4pt}
  \begin{tabular}{lcccccccccc}
    \toprule
    & \multicolumn{2}{c}{$w=1$} & \multicolumn{2}{c}{$w=2$} & \multicolumn{2}{c}{$w=4$} & \multicolumn{2}{c}{$w=6$} & \multicolumn{2}{c}{$w=8$} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
    & FID $\downarrow$ & CLIP $\uparrow$ & FID $\downarrow$ & CLIP $\uparrow$ & FID $\downarrow$ & CLIP $\uparrow$ & FID $\downarrow$ & CLIP $\uparrow$ & FID $\downarrow$ & CLIP $\uparrow$ \\
    \midrule
    \multicolumn{11}{l}{\textbf{Scale-RAE}} \\
    Baseline & 29.51 & \textbf{0.418} & 32.01 & \textbf{0.439} & 32.53 & \textbf{0.448} & 31.72 & \textbf{0.449} & 31.25 & \textbf{0.447} \\
    $t_0 = 0.02$ & 24.62 & 0.409 & 26.27 & 0.432 & 27.95 & 0.442 & 27.83 & 0.444 & 27.98 & 0.441 \\
    \rowcolor{gray!10}$t_0 = 0.05$ & \textbf{23.46} & 0.393 & \textbf{21.65} & 0.409 & \textbf{21.06} & 0.420 & \textbf{21.37} & 0.423 & \textbf{23.36} & 0.421 \\
    $t_0 = 0.1$ & 24.99 & 0.382 & 23.60 & 0.388 & 22.84 & 0.394 & 23.81 & 0.395 & 27.21 & 0.393 \\
    $t_0 = 0.2$ & 27.32 & 0.375 & 27.11 & 0.375 & 27.73 & 0.374 & 30.32 & 0.371 & 35.39 & 0.366 \\
    \midrule
    \multicolumn{11}{l}{\textbf{SVG-T2I}} \\
    Baseline & 23.05 & 0.369 & 20.55 & 0.420 & 22.30 & \textbf{0.440} & 23.31 & \textbf{0.445} & 23.73 & \textbf{0.447} \\
    $t_0 = 0.02$ & 18.73 & 0.388 & 18.49 & \textbf{0.423} & 21.08 & 0.439 & 22.55 & 0.443 & 23.30 & 0.444 \\
    \rowcolor{gray!10}$t_0 = 0.05$ & 16.22 & \textbf{0.390} & 16.04 & 0.412 & 16.96 & 0.430 & 17.88 & 0.438 & 18.56 & 0.441 \\
    $t_0 = 0.1$ & 15.54 & 0.389 & \textbf{15.23} & 0.401 & 15.44 & 0.414 & 15.72 & 0.421 & 16.02 & 0.425 \\
    $t_0 = 0.2$ & \textbf{15.33} & 0.387 & 15.25 & 0.391 & \textbf{15.29} & 0.397 & \textbf{15.34} & 0.401 & \textbf{15.59} & 0.404 \\
    \bottomrule
  \end{tabular}
\end{table*}

